Posterior linearisation smoothing with robust iterations

This paper considers the problem of iterative Bayesian smoothing in nonlinear state-space models with additive noise using Gaussian approximations. Iterative methods are known to improve smoothed estimates but are not guaranteed to converge, motivating the development of methods with better convergence properties. The aim of this article is to extend Levenberg-Marquardt (LM) and line-search versions of the classical iterated extended Kalman smoother (IEKS) to the iterated posterior linearisation smoother (IPLS). The IEKS has previously been shown to be equivalent to the Gauss-Newton (GN) method. We derive a similar GN interpretation for the IPLS and use this to develop extensions to the IPLS, with improved convergence properties. We show that an LM extension for the IPLS can be achieved with a simple modification of the smoothing iterations, enabling algorithms with efficient implementations. We also derive the Armijo--Wolfe step length conditions for the IPLS enabling an efficient inexact line-search method. Our numerical experiments show the benefits of these extensions in highly nonlinear scenarios.

==> alg/inexact_line_search.tex <==
\begin{algorithm}[t]
    \caption{Inexact Line Search IEKS}
    \label{alg:inexact_line_search}
    \small
    \begin{algorithmic}[1]
        \Require The initial trajectory $\hat{x}_{1:N}^0$, backtracking parameters $c_1,\tau$, and implicitly the measurements, model functions, Jacobians, and parameters: $z_{1:N}$, $f_{1:N}$, $h_{1:N}$, $F_{1:N}$, $H_{1:N}$, $Q_{1:N}$, $R_{1:N}$, $\hat{x}_1$, and $P_1$.
        \Ensure The MAP trajectory $\hat{x}_{1:N}^*$.
       \Procedure{GN-IEKS-ILS}{$\hat{x}_{1:N}^0,\tau$}\
        \State Set $i \gets 0$
        \Repeat
            \State $\hat{x}_{1:N}^{(i+1)} \gets \textsc{Reg-IEKS-Step}(\hat{x}_{1:N}^{(i)},0,\emptyset)$
            \State $\Delta \hat{x}_{1:N} \gets \hat{x}_{1:N}^{(i+1)} - \hat{x}_{1:N}^{(i)}$
            \State // Use Armijo backtracking to find admissible $\alpha$:
            \State $\alpha \gets 1$
%            \State $d \gets \textsc{Der}(\hat{x}_{1:N}^{(i)},\Delta \hat{x}_{1:N})$
            \State // Compute the directional derivative:
         \begin{equation*}
         \begin{split}
            d &\gets 2 \Delta \hat{x}_1^\top P_1^{-1} (\hat{x}_1^{(i)} - \hat{x}_1) \\
		  &+ 2 \sum_{k=2}^N (\Delta \hat{x}_k - F_{k-1}(\hat{x}_{k-1}^{(i)})
		  \Delta \hat{x}_{k-1})^\top \\
		&\qquad \times Q_{k-1}^{-1} (\hat{x}_k^{(i)} - f_{k-1}(\hat{x}_{k-1}^{(i)})) \\
  		&- 2 \sum_{k=1}^N (H_k(\hat{x}_k^{(i)}) \Delta \hat{x}_k)^\top
		R_k^{-1} (z_k - h_k(\hat{x}_k^{(i)}))
         \end{split}
         \end{equation*}
            \While{$L(\hat{x}_{1:N}^{(i)} + \alpha \Delta \hat{x}_{1:N}) \ge
                        L(\hat{x}_{1:N}^{(i)}) + \alpha c_1 d$}
              \State $\alpha \gets \tau \alpha$
            \EndWhile
            \State $\hat{x}_{1:N}^{(i+1)} \gets \hat{x}_{1:N}^{(i)} + \alpha \Delta \hat{x}_{1:N}$
            \State Set $i \gets i+1$
        \Until{Converged}
     \State \Return $\hat{x}_{1:N}^{(i)}$
     \EndProcedure
    \end{algorithmic}
\end{algorithm}


==> content/_our_method/derivation_gn_ipls.tex <==
\subsection{Proof of \cref{thm:gn_ipls:cost_fn:grad}}
\label{app:gn_ipls:grad}
The gradient of the \ipls cost function in \cref{eq:ipls:gn:cost_fn} is
\begin{align*}
  \grad \gnIplsObj{i}(\xSeq) &= \frac{1}{2} \twoNorm{\gnRIt{i}(\xSeq)}^2 \\
                             &= J_{\gnRIt{i}}(\xSeq)^{\top} \gnRIt{i}(\xSeq).
\end{align*}

To compute $J_{\gnRIt{i}}(\xSeq)$, where $\gnRIt{i}$ is defined in \cref{eq:def:ipls:gnr},
we need the Jacobians of the \slr expectations $\stateBar(\cdot), \measBar(\cdot)$
(for brevity we use the shorthand $p_{\ts}(\x) = \normal(\x; \x_{\ts}, \PHatIt{i}_{\ts})$):
\begin{small}
\begin{align}
  \label{eq:ipls:proc_jacobian}
  J_{\stateBar_{\ts}}(\x_{\ts}) &= J(\expect{\procFn(\x_{\ts})}) \nonumber \\
                                &= J \left( \int \procFn(\x) p_{\ts}(\x) \d \x \right) \nonumber \\
                                &= \int \procFn(\x) J(p_{\ts}(\x)) \d \x \nonumber \\
                                &= \int \procFn(\x) (\x - \x_{\ts})^{\top} p_{\ts}(\x) \d \x \PHatItInv{i}
\end{align}
\end{small}
Here, we use equation (S-9 in \cite{damped_plf}) and note that
\begin{small}
\begin{align}
  \label{eq:ipls:zero_int}
  \int &\stateBar_{\ts}(\x_{\ts}) \left( \x - \x_{\ts} \right)^{\top} p_{\ts}(\x) \d \x \nonumber \\
       &= \stateBar_{\ts}(\x_{\ts}) \left( \int \x^{\top}  p_{\ts}(\x) \d \x - \x_{\ts}^{\top}  \int p_{\ts}(\x) \d \x \right) \nonumber \\
       &= \stateBar_{\ts}(\x_{\ts}) \left( \x_{\ts}^{\top}- \x_{\ts}^{\top} \right)
       = 0.
\end{align}
\end{small}
We substitute \cref{eq:ipls:zero_int} into the derivative in \cref{eq:ipls:proc_jacobian} to obtain
\begin{align}
  \label{eq:ipls:proc_bar:deriv}
  &J_{\stateBar_{\ts}}(\x_{\ts}) \nonumber \\
  &= \int \left( \procFn(\x) - \stateBar_{\ts}(\x_{\ts}) \right) \left( \x - \x_{\ts} \right)^{\top} p_{\ts}(\x) \d \x\ \PHatItInv{i}\nonumber \\
  &= \PsiSlr{\procFn_{\ts}}^{\top}(\x_{\ts}) \PHatItInv{i} = \procAIt{i}_{\ts}(\x_{\ts}),
\end{align}
i.e., the \slr Jacobian in \cref{eq:slr:jacobian}, based on the estimates at iteration $i$.

Analogously,
\begin{align}
  \label{eq:ipls:meas_bar:deriv}
  J_{\measBar_{\ts}}(\x_{\ts}) = \PsiSlr{\measFn_{\ts}}^{\top}(\x_{\ts}) \PHatItInv{i} = \measHIt{i}_{\ts}(\x_{\ts})
\end{align}
%
Given the definition of $\gnRIt{i}$ in \cref{eq:def:ipls:gnr}, let $\allDim = \tsFin \dimState + \tsFin \dimMeas$ and compute the Jacobian $J_{\gnRIt{i}}(\xSeq): \reals^{\tsFin \dimState} \to \reals^{\allDim \times \tsFin \dimState}$, in terms of the above Jacobians:
\begin{align}
  \label{eq:ipls:gnr:jacobian}
  J_{\gnRIt{i}}(\xSeq) &= J_{\augQIplsInvSqrtT \augObsIpls}(\xSeq)
  = \augQIplsInvSqrtT J_{\augObsIpls}(\xSeq) \nonumber \\
              &= \augQIplsInvSqrtT
              \begin{pmatrix}
                \procAIt{i}(\xSeq)\\
                \measHIt{i}(\xSeq)
              \end{pmatrix}
\end{align}
where,
\begin{align}
  \label{eq:def:ipls:proc_jacobian_seq}
  &\procAIt{i}(\xSeq) \coloneqq \nonumber \\
  &\begin{pmatrix}
    I_{\dimState} &0 &\hdots &~ &~ &0 \\
    -\procAIt{i}_1(\x_1) &I_{\dimState} &0 &~ &\hdots &0 \\
    0 &-\procAIt{i}_2(\x_2) &I_{\dimState} &0 &\hdots &0 \\
    \vdots &~ &\ddots &\ddots &~ &\vdots \\
    0 &~ &\dots &~ &I_{\dimState} &0 \\
    0 &~ &\dots &~ & -\procAIt{i}_{\tsFin-1}(\x_{\tsFin-1}) &I_{\dimState}\\
  \end{pmatrix} \nonumber \\
\end{align}
and
\begin{align}
  \label{eq:def:ipls:meas_jacobian_seq}
  \measHIt{i}(\xSeq) \coloneqq - \diag \left( \measHIt{i}_1(\x_1), \measHIt{i}_2(\x_2), \dots, \measHIt{i}It{i}_{\tsFin}(\x_{\ts}) \right).
\end{align}

\subsection{Proof details of \cref{thm:gn_ipls}}
\label{app:gn_ipls}
The proof of \cref{thm:gn_ipls} has a similar structure as the proof of \cref{thm:gn_ieks},
which is outlined in \cref{fig:props_overview}.
The proof requires linearising and construction of the approximative GN cost function $\gnRLin$
and \slr linearisation of the state-space model in \cref{eq:def:state_space_model}.
We then show that that this approximate GN objective corresponds to this approximate state-space model.
Here, we provide details of these steps.

The important part of the linearisation comes from \cref{thm:gn_ipls:cost_fn:grad}.
From the Jacobian $J_{\gnRIt{it}}$ we make the \gn approximation,
linearising around the current smoothed state sequence estimate $\xHatItSeq{i}$:
%\begin{scriptsize}
\begin{align}
  \label{eq:app:ipls:gnr:taylor}
  &\gnRIt{i}(\xSeq) \approx \gnRLin(\xSeq) = \gnRIt{i}(\xHatItSeq{i}) + J_{\gnRIt{i}}(\xHatItSeq{i}) (\xSeq - \xHatItSeq{i}) \nonumber \\
             &= \augQIplsInvSqrtT \augObsIpls(\xHatItSeq{i}) \nonumber \\
             &+ \augQIplsInvSqrtT
             \begin{pmatrix}
               \procAIt{i}(\xHatItSeq{i}) \\
               \measHIt{i}(\xHatItSeq{i})
             \end{pmatrix}
             (\xSeq - \xHatItSeq{i}) \nonumber \\
             % &= \augQIplsInvSqrtT \nonumber \\
             % &\begin{pmatrix}
             %   \xHatIt{i}_1 - \priorMean + \x_1 - \xHatIt{i}_1\\
             %   \xHatIt{i}_2 - \stateBar_1(\xHatIt{i}_1) - \procAIt{i}_{1}(\xHatIt{i}_1) (\x_1 - \xHatIt{i}_1) + (\x_2 - \xHatIt{i}_2)\\
             %   \xHatIt{i}_3 - \stateBar_2(\xHatIt{i}_2) - \procAIt{i}_{2}(\xHatIt{i}_2) (\x_2 - \xHatIt{i}_2) + (\x_3 - \xHatIt{i}_3)\\
             %   \vdots \\
             %   \xHatIt{i}_{\tsFin} - \stateBar_{\tsFin - 1}(\xHatIt{i}_{\tsFin - 1}) - \procAIt{i}_{\tsFin-1}(\xHatIt{i}_{\tsFin-1}) (\x_{\tsFin-1} - \xHatIt{i}_{\tsFin-1}) + (\x_{\tsFin} - \xHatIt{i}_{\tsFin})\\
             %   \meas_1 - \measBar_1(\xHatIt{i}_1) - \measHIt{i}_{1}(\xHatIt{i}_1) (\x_1 - \xHatIt{i}_1)\\
             %   \meas_2 - \measBar_2(\xHatIt{i}_2) - \measHIt{i}_{2}(\xHatIt{i}_2) (\x_2 - \xHatIt{i}_2)\\
             %   \vdots \\
             %   \meas_{\tsFin} - \measBar_{\tsFin}(\xHatIt{i}_{\tsFin}) - \measHIt{i}_{{\tsFin}}(\xHatIt{i}_{\tsFin}) (\x_{\tsFin} - \xHatIt{i}_{\tsFin})\\
             % \end{pmatrix} \nonumber \\
             &= \augQIplsInvSqrtT
             \underbrace{
             \begin{pmatrix}
               \x_1 - \priorMean \\
               \x_2 - \left( \procAIt{i}_{1}(\xHatIt{i}_1) \x_1 + \procB_{1}(\xHatIt{i}_1) \right ) \\
               \x_3 - \left( \procAIt{i}_{2}(\xHatIt{i}_2) \x_2 + \procB_{2}(\xHatIt{i}_2) \right ) \\
               \vdots \\
               \x_{\tsFin} - \left( \procAIt{i}_{\tsFin-1}(\xHatIt{i}_{\tsFin}) \x_{\tsFin} + \procB_{\tsFin-1}(\xHatIt{i}_{\tsFin}) \right ) \\
               \meas_1 - \left( \measHIt{i}_{1}(\xHatIt{i}_1) \x_1 + \measC_{1}(\xHatIt{i}_1) \right) \\
               \vdots \\
               \meas_{\tsFin} - \left( \measHIt{i}_{\tsFin}(\xHatIt{i}_{\tsFin}) \x_{\tsFin} + \measC_{\tsFin}(\xHatIt{i}_{\tsFin}) \right) \\
             \end{pmatrix}}_{\coloneqq \augObsIplsApprox(\xSeq)} \nonumber \\
             &= \augQIplsInvSqrtT \augObsIplsApprox(\xSeq)
\end{align}
%\end{scriptsize}
% where, in the second to last equality, we use the relation in \cref{eq:slr:offset}, that is, $\stateBar(\xHatIt{i}_{\ts}) - \procAIt{i}_{\ts}(\xHatIt{i}_{\ts}) \xHatIt{i}_{\ts} = \procB_{\ts}(\xHatIt{i}_{\ts})$.
% Analogously for the \slr linearisation of $\measFn(\cdot)$.
where, in the second to last equality, we use the relation in \cref{eq:slr:offset} to express $\gnRLin(\xSeq)$ in terms of the offsets $\procB_{1:\tsFin}(\cdot)$ and $\measC_{1:\tsFin}(\cdot)$.


==> content/_our_method/gn_ipls.tex <==
\subsection{\gn cost function}
\label{sec:our_method:ipls}
\noindent Inspired by the \ieks, we seek to establish a similar connection between the \ipls and the \gn method.
To this end, we require a cost function that leads to a \gn method, corresponding to the \ipls.

A key difference between the \ieks and the \ipls is the role the covariances play.
In the \ieks, the analytical linearisation is done only with respect to the estimated means $\xHatItSeq{i}$, whereas the \slr linearisation of the \ipls is based on both the estimated means $\xHatItSeq{i}$ and covariances $\PHatItSeq{i}$.
The \ieks further assumes that the linearisation error covariances are zero, whereas the \ipls estimates them as $\procLinCovIt{i}_{\ts}$ and $\measLinCovIt{i}_{\ts}$ respectively.
These matrices appear in the approximate state-space model of \cref{eq:def:lin:state_space_model} and must therefore be included in a cost function.
The estimated covariances $\PHatItSeq{i}$ are implicitly included in the approximate state-space model, since they are used in the \slr linearisation.

The inclusion of the covariance matrices complicates the construction of a matching \gn objective, which should be on a quadratic form in the state sequence $\xSeq$ (or some function of it).
Note that the state sequence $\xSeq$ is the optimisation variable and that the solution to the optimisation problem becomes the state estimates $\xHatItSeq{i+1}$.
The matrix defining the quadratic form will depend on the (estimated means of the) state sequence $\xHatItSeq{i}$ and the cost function will also, implicitly, depend on the covariance sequence $\PHatItSeq{i}$.

To establish the link between the \gn method and \ipls, we construct a cost function for the sequence of states fixing the covariances $\procLinCovIt{i}_{1:\tsFin}$, $\measLinCovIt{i}_{1:\tsFin}$ and $\PHatItSeq{i}$:
\begin{align}
  \label{eq:ipls:gn:cost_fn}
  &\gnIplsObj{i}(\xSeq) \nonumber \\
  &= \frac{1}{2} \Big( (\x_1 - \priorMean)^{\top} \priorCov^{-1} (\x_1 - \priorMean) \nonumber \\
  &+ \sum_{\ts=1}^{\tsFin-1} (\x_{\ts+1} - \stateBar_{\ts}(\x_{\ts}))^{\top} \left(\procCov_{\ts} + \procLinCovIt{i}_{\ts} \right)^{-1} (\x_{\ts+1} - \stateBar_{\ts}(\x_{\ts})) \nonumber \\
  &+ \sum_{\ts=1}^\tsFin (\meas_{\ts} - \measBar_{\ts}(\x_{\ts}))^{\top} \left( \measCov_{\ts} + \measLinCovIt{i}_{\ts} \right)^{-1} (\meas_{\ts} - \measBar_{\ts}(\x_{\ts})) \Big),
\end{align}
where $\stateBar(\cdot), \measBar(\cdot)$ are
%calculated as in \cref{eq:slr:z_bar}, but restated here for clarity
the \slr estimated expectations:
\begin{subequations}
\begin{align}
  \label{eq:ipls:state_bar}
  \stateBar_{\ts}(\x_{\ts}) &= \int \procFn_{\ts}(\x) \normal(\x; \x_{\ts}, \PHatIt{i}_{\ts}) \d \x,\\
  \label{eq:ipls:meas_bar}
  \measBar_{\ts}(\x_{\ts}) &= \int \measFn_{\ts}(\x) \normal(\x; \x_{\ts}, \PHatIt{i}_{\ts}) \d \x,
\end{align}
\end{subequations}
% Same line to avoid a space indent
and $\procLinCovIt{i}_{\ts}, \measLinCovIt{i}_{\ts}$ are computed using \cref{eq:slr:cov} with respect to $\xHatItSeq{i}, \PHatItSeq{i}$ using $\procFn_{\ts}$ and $\measFn_{\ts}$ in \cref{eq:slr:moments} respectively.

An important property is that the cost function in \cref{eq:ipls:gn:cost_fn} depends on the most recent estimate of the sequence of covariance matrices,
both through the \slr expectations in \cref{eq:ipls:state_bar,eq:ipls:meas_bar} and through the estimated linearisation errors $\procLinCovIt{i}_{\ts}$ and $\measLinCovIt{i}_{\ts}$.

\input{content/our_method/gn_ipls_thm.tex}
% \input{content/our_method/gn_ipls_interpret.tex}


==> content/_our_method/gn_ipls_interpret.tex <==
It is important to note that fixing the covariance sequence does not restrict the \rts smoother's solution of the approximate problem.
The previous estimates only affect the linearisation of the state-space model, which is always fixed during the actual smoothing pass, regardless of cost function.
The effect is only present across iterations where the method essentially requires a design-choice; keeping the same covariance sequence and cost function,
or updating the covariances, thereby changing to the next optimisation objective in the sequence.

By keeping $\procLinCovIt{i}_{\ts}, \measLinCovIt{i}_{\ts}$ fixed, we perform proper \gn optimisation for a cost function in the sequence.
A specific cost function in the sequence can be optimised multiple times, creating a sequence of intermediate estimates of the means sequence. When this ``inner'' loop is finished, we obtain the estimates $\xHatItSeq{i+1}, \PHatItSeq{i+1}$,
and move on to the next cost function in the sequence.

The update has two effects: it explicitly updates the estimated covariances of the linearisation errors,
and implicitly alters the \slr expectations $\stateBar, \measBar$, see \cref{eq:slr:moments}.
The method we propose allows for the choice between the two extremes of updating to the next cost function at every iteration or optimising each cost function to convergence before updating the covariances, or indeed something in between, with some arbitrary stopping criterion.


==> content/_our_method/gn_ipls_thm.tex <==
Before we derive the connection between \gn and \ipls we need to derive an expression for the gradient of our proposed cost function.
\begin{lemma}
  \label[lemma]{thm:gn_ipls:cost_fn:grad}
  The gradient of the \ipls cost function in \cref{eq:ipls:gn:cost_fn} is
  \begin{align}
    \label{eq:ipls:gn:cost_fn:grad}
    &\grad \gnIplsObj{i}(\xSeq) = J_{\gnRIt{i}}(\xSeq)^{\top} \gnRIt{i}(\xSeq),
  \end{align}
  where,
  \begin{align}
  J_{\gnRIt{i}}(\xSeq)^{\top}% \nonumber \\
  &= \begin{pmatrix}
    (\procAIt{i}(\xSeq))^{\top} & (\measHIt{i})(\xSeq))^{\top}
  \end{pmatrix} \augQIplsInvSqrt.
  \end{align}
\end{lemma}
where $\procAIt{i}(\xSeq)$ and $\measHIt{i}(\xSeq)$ are given by
\cref{eq:def:ipls:proc_jacobian_seq} and \cref{eq:def:ipls:meas_jacobian_seq} in the supplementary material,
which also contains the proof of \cref{thm:gn_ipls:cost_fn:grad}.

We can then go on to present the main result of this section.
\begin{prop}
  \label[prop]{thm:gn_ipls}
The output of one iteration of \gn optimisation of the cost function $\gnIplsObj{i}(\xSeq)$ in \cref{eq:ipls:gn:cost_fn}, defined by the current \gn estimate $\xHatItSeq{i}$ and the covariance matrices $\PHatItSeq{i}$, is the same as the means estimated by \rts smoothing of \cref{eq:def:state_space_model}, linearised with \slr around $\xHatItSeq{i}, \PHatItSeq{i}$, that is, one iteration of the \ipls.
%With $\PHatIt{i}_{\ts}, \procLinCovIt{i}_{\ts}, \measLinCovIt{i}_{\ts}$ fixed for all $k = 1, \dots, \tsFin$,
%\ipls inference of the state-space model in \cref{eq:def:state_space_model} is a \gn method for minimising the cost function in \cref{eq:ipls:gn:cost_fn}.
\end{prop}

\begin{proof}
The proof follows the steps outlined in \cref{fig:props_overview}.
We construct $\gnRIt{i}(\xSeq)$ such that $\gnIplsObj{i}(\xSeq) = \frac{1}{2} \twoNorm{\gnRIt{i}(\xSeq)}^2$ and then linearise $\gnRIt{i}(\xSeq)$ to form the approximate objective $\gnIplsObjLin{i}(\xSeq)$.
Secondly, the state-space model is linearised with \slr, according to the \ipls.
Finally, we compare the approximate \gn objective to the linearised state-space model and note that they correspond to the same minimisation problem.

Note that the covariance matrices $\procLinCovIt{i}_{\ts}$ and $\measLinCovIt{i}_{\ts}$ in $\gnIplsObj{i}(\xSeq)$ depend on the current estimates $\xHatItSeq{i}$ and not on the optimisation variable $\xSeq$.
Therefore, $\gnIplsObj{i}(\xSeq)$ is on the form of \cref{eq:gn:problem_form} and can be optimised with the \gn method.

We construct $\gnRIt{i}(\xSeq)$ by collecting states and measurements in a vector and group the covariance matrices in a single block diagonal matrix:
\begin{subequations}
\begin{align}
  \label{eq:def:ipls:aug_obs}
  \augObsIpls(\xSeq) &= \begin{pmatrix}
    \x_1 - \priorMean \\
    \x_2 - \stateBar_1(\x_1) \\
    \vdots \\
    \x_{\tsFin} - \stateBar_{\tsFin-1}(\x_{\tsFin-1}) \\
    \meas_1 - \measBar_1(\x_1) \\
    \meas_2 - \measBar_2(\x_2) \\
    \vdots \\
    \meas_{\tsFin} - \measBar_{\tsFin}(\x_{\tsFin})
  \end{pmatrix}, \\
  \label{eq:def:ipls:augQ}
  \augQIplsInv &= \diag \Big( \nonumber \\
  &\priorCov^{-1}, (\procCov_1 + \procLinCovIt{i}_1)^{-1}, \dots, (\procCov_{\tsFin-1} + \procLinCovIt{i}_{\tsFin-1})^{-1},\nonumber \\
                 &(\measCov_1 + \measLinCovIt{i}_1)^{-1}, \dots, (\measCov_{\tsFin} + \measLinCovIt{i}_{\tsFin})^{-1} \Big).
\end{align}
\end{subequations}
Defining
\begin{equation}
  \label{eq:def:ipls:gnr}
  \gnRIt{i}(\xSeq) = \augQIplsInvSqrtT \augObsIpls(\xSeq),
\end{equation}
with $\augQIplsInvSqrt \augQIplsInvSqrtT = \augQIplsInv$, we confirm that
\begin{equation*}
  %\label{eq:ipls:cost_compact}
  \frac{1}{2} \twoNorm{\gnRIt{i}(\xSeq)}^2 = \augObsIpls^{\top}(\xSeq) \augQIplsInv \augObsIpls(\xSeq) = \gnIplsObj{i}(\xSeq).
\end{equation*}

Next, we linearise $\gnRIt{i}$ by computing the first-order approximation around $\xHatItSeq{i}$
\begin{align}
  \label{eq:ipls:gnr:taylor}
  &\gnRIt{i}(\xSeq) \approx \gnRLin(\xSeq) \nonumber \\
             &= \gnRIt{i}(\xHatItSeq{i}) + J_{\gnRIt{i}}(\xHatItSeq{i}) (\xSeq - \xHatItSeq{i}) \nonumber \\
             &= \augQIplsInvSqrtT \augObsIpls(\xHatItSeq{i})
             + \augQIplsInvSqrtT J_{\augObsIpls}(\xSeq)(\xSeq - \xHatItSeq{i}) \nonumber \\
             &= \augQIplsInvSqrtT \augObsIplsApprox(\xSeq),
\end{align}
where
\begin{align*}
  &\augObsIplsApprox(\xSeq) = \nonumber \\
                      &\begin{pmatrix}
               \x_1 - \priorMean \\
               \x_2 - \left( \procAIt{i}_1(\xHatIt{i}_1) \x_1 + \procB_{1}(\xHatIt{i}_1) \right ) \\
               \x_3 - \left( \procAIt{i}_{2}(\xHatIt{i}_2) \x_2 + \procB_{2}(\xHatIt{i}_2) \right ) \\
               \vdots \\
               \x_{\tsFin} - \left( \procAIt{i}_{\tsFin-1}(\xHatIt{i}_{\tsFin-1}) \x_{\tsFin-1} + \procB_{\tsFin-1}(\xHatIt{i}_{\tsFin-1}) \right ) \\
               \meas_1 - \left( \measHIt{i}_{1}(\xHatIt{i}_1) \x_1 + \measC_{1}(\xHatIt{i}_1) \right) \\
               \vdots \\
               \meas_{\tsFin} - \left( \measHIt{i}_{\tsFin}(\xHatIt{i}_{\tsFin}) \x_{\tsFin} + \measC_{\tsFin}(\xHatIt{i}_{\tsFin}) \right) \\
             \end{pmatrix}
\end{align*}
and $\procAIt{i}_{\ts}(\x_{\ts}), \measHIt{i}_{\ts}(\x_{\ts})$ are the \slr Jacobians of $\procFn_{\ts}, \measFn_{\ts}$ respectively,
see the supplementary material for the derivation details.

The approximate \gn objective becomes
\begin{align}
  \label{eq:ipls:approx_objective}
  &\gnIplsObjLin{i}(\xSeq) \nonumber \\
  % = \frac{1}{2} \twoNorm{ \gnRLin(\xSeq) }^2
  &= \frac{1}{2}\left(\augObsIplsApprox(\xSeq)\right)^{\top} \augQIplsInv \augObsIplsApprox(\xSeq) \left(\augObsIplsApprox(\xSeq)\right).
\end{align}
%We defined $\gnIplsObj{i}(\xSeq)$ in terms of the current estimates $\xHatItSeq{i}, \PHatItSeq{i}$.
%The next \gn iterate $\xHatItSeq{i}$ is the estimate that exactly minimises $\gnIplsObjLin{i}(\xSeq)$.
To perform one iteration of \ipls, we instead first linearise the state-space model in \cref{eq:def:state_space_model} using \slr with respect to $\normal(\x_{\ts}; \xHatIt{i}_{\ts}, \PHatIt{i}_{\ts})$.
The resulting approximate state-space model is on the form \cref{eq:def:lin:state_space_model} with linearisation parameters $\affAppParam{i}$ selected using \cref{eq:slr:jacobian,eq:slr:offset,eq:slr:cov}.
The next iterate $\xHatItSeq{i+1}$ is computed as the closed-form output of \rts smoothing.

Examining $\gnIplsObjLin{i}(\xSeq)$, we note that it is the negative log-posterior of the \slr linearised state-space model (up to a constant).
The next \gn iterate will be the closed-form solution to this minimisation problem.
Since the two methods, \gn and \ipls, in a single iteration computes the exact solution to the same optimisation problem, their output $\xHatItSeq{i+1}$ must be the same.
\end{proof}


==> content/_our_method/line_search.tex <==
\section{Line-search}
\label{sec:our_method:line_search}
\noindent Another way to improve the \gn method is to introduce a line-search procedure to the algorithm \cite{num_opt}. The line-search version of the \ieks was described in \cite{lm_ieks} and here we extend it to the \ipls.
Line-search can be implemented by introducing a parameter $\alpha > 0$ to restrict the iterative update of the estimates.
That is, given $\xHatItSeq{i+1}$ and $\xHatItSeq{i}$,
we define $\searchDirSeq{i} = \xHatItSeq{i+1} - \xHatItSeq{i}$, and we obtain the line-search update of the estimates:
\begin{equation}
  \label{eq:ls:update}
  \xHatItSeq{i+1}(\alpha) = \xHatItSeq{i} + \alpha \searchDirSeq{i}% \nonumber \\
  %\PHatItSeq{i+1}(\alpha) &= \PHatItSeq{i} + \alpha \Delta \PHatItSeq{i+1},
\end{equation}
where
\begin{equation}
  \label{eq:ls:step_length}
  \alpha = \argMin{\alpha' \in [0,1]} \gnObj^{(i)}(\xHatItSeq{i} + \alpha' \searchDirSeq{i}).
\end{equation}

We can also use an inexact version of line-search, where we seek a point
$\lsPoint = \xHatItSeq{i} + \alpha \searchDirSeq{i}$,
for which we only require a sufficient decrease in the cost function.
This is guaranteed by fulfilling the Armijo or Wolfe conditions \cite{num_opt}
\begin{subequations}
\begin{align}
  \label{eq:def:armijo_cond}
  \costFn(\lsPoint) \leq \costFn(\xHatItSeq{i}) + c_1 \alpha (\searchDirSeq{i})^{\top} \grad \costFn(\xHatItSeq{i}) \\
  \label{eq:def:wolfe_cond}
  (\searchDirSeq{i})^{\top} \grad \costFn(\lsPoint) \geq c_2 (\searchDirSeq{i})^{\top} \grad \costFn(\xHatItSeq{i}),
\end{align}
\end{subequations}
where $0 < c_1 < c_2 < 1$.

\begin{lemma}
  \label[lemma]{thm:ls:armijo_wolfe:ipls}
  An efficient computation of the directional derivatives for the \ipls cost function in \cref{eq:ipls:gn:cost_fn} to evaluate the Armijo--Wolfe conditions in \cref{eq:def:armijo_cond,eq:def:wolfe_cond}
  is given by
  \begin{align}
    &(\searchDirSeq{i})^{\top} \grad \costFn(\xHatItSeq{i}) \nonumber \\
    &= (\searchDir{i}_{1})^{\top} \priorCov^{-1}(\xHatIt{i}_1 - \priorMean) \nonumber \\
    &+ \sum_{\ts=1}^{K-1} \left( \searchDir{i}_{\ts+1} - \procA_{\ts}(\xHatIt{i}_\ts) \searchDir{i}_{\ts} \right)^{\top} \nonumber \\
    &\hspace{1cm} \times (\procCov_{\ts} + \procLinCovIt{i}_{\ts})^{-1}(\xHatIt{i}_{\ts+1} - \stateBar_\ts(\xHatIt{i}_\ts)) \nonumber \\
    &- \sum_{\ts=1}^{K} \left( \measH_{\ts}(\xHatIt{i}_\ts) \searchDir{i}_{\ts} \right)^{\top} (\measCov_{\ts} + \measLinCovIt{i}_{\ts})^{-1}(\xHatIt{i}_{\ts+1} - \measBar_\ts(\xHatIt{i}_\ts)). \nonumber \\
  \end{align}
\end{lemma}
\begin{proof}
To evaluate the Armijo--Wolfe conditions for a certain step length $\alpha$,
we need to compute the gradient of the cost function in \cref{eq:ipls:gn:cost_fn},
which comes directly from \cref{thm:gn_ipls:cost_fn:grad}.

The derivations of the directional derivatives are in the supplementary material.
\end{proof}

By selecting a suitable estimate on a line between the previous estimate and the new one proposed by the smoothing iteration,
the methods improve, since the size of the update step is allowed to decrease for iteration updates that risk diverging.
Potentially, this could also lead to faster convergence, albeit with the extra computational demand incurred by finding a suitable $\alpha$.


==> content/_our_method/line_search_conditions.tex <==
\subsection{Armijo and Wolfe step length conditions}
% TODO: pT grad f not guranteed to be negative.
This section provides the Armijo and Wolfe step length conditions for the LS-IPLS method, see \cref{eq:def:armijo_cond,eq:def:wolfe_cond}.
An inexact line-search method only requires a sufficient decrease in the cost function, rather than finding the minimum along the search direction $\searchDirSeq{i}$.
A sufficient decrease is guaranteed by fulfilling two conditions of the cost function and its gradient at a point on the line.

The first condition is commonly referred to as the Armijo condition,
and combined they are called the Wolfe conditions or the Armijo--Wolfe conditions\cite{num_opt}.
The Armijo condition is a sufficient condition for a decreasing cost function,
whereas the Wolfe condition ensures that the step length $\alpha$ is large enough to give faster convergence.

To check the Armijo--Wolfe conditions for a certain step length $\alpha$ we need to compute the gradient of the cost function,
which comes directly from \cref{thm:gn_ipls:cost_fn:grad}.

Due to the sparseness of the Jacobian, the directional derivative can be computed more efficiently by evaluating the product
\begin{align}
  &(\searchDirSeq{i})^{\top} \grad \costFn(\xHatItSeq{i}) \nonumber \\
  &= (\searchDir{i}_{1})^{\top} \priorCov^{-1}(\xHatIt{i}_1 - \priorMean) \nonumber \\
  &+ \sum_{\ts=1}^{K-1} \left( \searchDir{i}_{\ts+1} - \procA_{\ts}(\xHatIt{i}_\ts) \searchDir{i}_{\ts} \right)^{\top} \nonumber \\
  &\hspace{1cm} \times (\procCov_{\ts} + \procLinCovIt{i}_{\ts})^{-1}(\xHatIt{i}_{\ts+1} - \stateBar_\ts(\xHatIt{i}_\ts)) \nonumber \\
  &- \sum_{\ts=1}^{K} \left( \measH_{\ts}(\xHatIt{i}_\ts) \searchDir{i}_{\ts} \right)^{\top} (\measCov_{\ts} + \measLinCovIt{i}_{\ts})^{-1}(\xHatIt{i}_{\ts+1} - \measBar_\ts(\xHatIt{i}_\ts)). \nonumber \\
\end{align}

The derivations for the gradient of the \ieks cost function are analogous,
but instead using the actual measurement and motion models and their respective analytical Jacobians.


==> content/_our_method/lm_reg_thm.tex <==
\subsection{Levenberg--Marquardt regularisation}
\label{sec:our_method:lm}
\noindent The now established connection between the \ieks and \ipls and \gn optimisation makes the \lm method a promising alternative for regularisation.
\Cref{thm:lm_rts_smoothing} shows how \lm-regularisation can be achieved through smoothing of a slightly modified state-space model.
The result was shown for the \lmIeks in \cite{lm_ieks} and is here generalised to include the \lmIpls.
Similar interpretations of regularisation as extra measurements are discussed in \cite{lm_ieks_2,lm_observation},
but only for the \ieks.
%
\begin{prop}
  \label[prop]{thm:lm_rts_smoothing}
  Iterated smoothing with \ieks or \ipls (under the conditions in \cref{thm:gn_ipls}) for a state-space model as in \cref{eq:def:state_space_model}, extended with the measurement
  \begin{equation}
    \label{eq:lm:extended_problem}
    \xHatIt{i}_{\ts} = \x_{\ts} + \lmErr_{\ts},\qquad \lmErr_{\ts} \sim \normal(0, (\lmRegParamIt{i})^{-1} \regMat^{(i)}_{\ts})
  \end{equation}
  is a \gn method with the \lm-regularisation defined in \cref{eq:lm:cost_fn}, if $\regMat^{(i)}$ is a sequence of block-diagonal regularisation matrices:
  $\regMat^{(i)} = \diag(\regMat_1^{(i)}, \dots, \regMat_{\tsFin}^{(i)}),\, \regMat^{(i)}_{\ts} \in \reals^{\dimState \times \dimState}, \forall \ts = 1, \dots, \tsFin$.
\end{prop}

\begin{proof}
The proof follows the structure of the earlier proofs and we can use the results of \cref{thm:gn_ieks,thm:gn_ipls} to simplify it.
First, we construct $\gnRLM{i}(\xSeq)$ such that $\lmObj{i}(\xSeq) = \frac{1}{2} \twoNorm{\gnRLM{i}(\xSeq)}^2$ and
show that the linearisation of $\gnRLM{i}(\xSeq)$ results in an approximate objective which is $\gnObjLin(\xSeq)$ plus an extra term.
Second, we introduce the measurement in \cref{eq:lm:extended_problem} into the state-space model \cref{eq:def:state_space_model} and linearise.
Third, we confirm that the \lm optimisation and iterative smoothers solve the same minimisation problem at each iteration.

In step 1 we derive the approximate \lm objective.
From \cref{eq:lm:cost_fn} we have that the \lm objective $\lmObj{i}(\xSeq)$ is the sum of the \gn objective $\gnObj(\xSeq)$ and a regularisation term.
By simply extending $\gnR(\xSeq)$ in \cref{eq:def:ipls:gnr}, we can construct
\begin{align}
  \label{eq:def:ipls:lm:gnr}
  \gnRLM{i}(\xSeq) &=
  \begin{pmatrix}
    \gnR(\xSeq) \\
    \lmRegSqrtT (\xSeq - \xHatItSeq{i})
  \end{pmatrix},
\end{align}
such that $\lmObj{i}(\xSeq) = \frac{1}{2}\twoNorm{\gnRLM{i}}^2$.

Since the regularisation term is linear in $\xSeq$, the resulting linearisation is
\begin{align}
  \gnRLM{i}(\xSeq) \approx
  \begin{pmatrix}
    \gnRLin(\xSeq) \\
    \lmRegSqrtT (\xSeq - \xHatItSeq{i})
  \end{pmatrix},
\end{align}
where we note that the approximate objective is indeed the approximate \gn objective in \cref{eq:ipls:approx_objective} with added \lm regularisation
\begin{align}
  \label{eq:ipls:lm:approx_cost}
  &\lmObjLin(\xSeq) \nonumber \\
  &= \frac{1}{2}
  \twoNorm{
  \begin{pmatrix}
    \gnRLin(\xSeq) \\
    \lmRegSqrtT (\xSeq - \xHatItSeq{i})
  \end{pmatrix}
  }^2
  \nonumber \\
                   &= \gnObjLin(\xSeq) \nonumber \\
                   &+ \frac{1}{2} \lmRegParamIt{i} (\xSeq - \xHatItSeq{i})^{\top} \left[ \regMat^{(i)}\right]^{-1} (\xSeq - \xHatItSeq{i}).
\end{align}

In step 2 we derive the negative log-posterior for the linearised state-space model with the measurement $\xHatIt{i}_{\ts}$ in \cref{eq:lm:extended_problem}.
The additional measurement will, for each timestep, contribute with a term $\frac{1}{2} \lmRegParamIt{i} (\x_{\ts} - \xHatIt{i}_{\ts})^{\top} \left[ \regMat^{(i)}_{\ts}\right]^{-1} (\x_{\ts} - \xHatIt{i}_{\ts})$ to the negative log-posterior.
All the extra measurements can be combined into a single term $\frac{1}{2} \lmRegParamIt{i} (\xSeq - \xHatItSeq{i})^{\top} \left[ \regMat^{(i)}\right]^{-1} (\xSeq - \xHatItSeq{i})$,
with the block-diagonal matrix $\regMat^{(i)} = \diag(\regMat_1^{(i)}, \regMat_2^{(i)}, \dots, \regMat_{\tsFin}^{(i)}),\, \regMat^{(i)}_{\ts} \in \reals^{\dimState \times \dimState}$.
Note that we restrict ourselves to $\regMat^{(i)}$ on this form, whereas other suitable options exist \cite{num_opt,nonlinear_regression}.
The measurement model for $\xHatItSeq{i}$ is linear in $\xSeq$ so the negative log-posterior of the approximated state-space model produced by \ieks or \ipls linearisation will be extended with this term.
%Compared to the previous posterior, this additional measurement will give rise to a term $\frac{1}{2} \lmRegParamIt{i} (\xSeq - \xHatItSeq{i})^{\top} \left[ \regMat^{(i)}\right]^{-1} (\xSeq - \xHatItSeq{i})$.
%For the particular choice of a sequence of block-diagonal regularisation matrices in the propostion formulation
%$\xHatItSeq{i}$ can be interpreted as a measurement of normally distributed $\xSeq$ with noise covariance $(\lmRegParamIt{i}^{-1}) \regMat^{(i)}_{\ts}$ (for every timestep $\ts$) as in \cref{eq:lm:extended_problem}.

In step 3 we compare the linearisations.
We know from \cref{thm:gn_ieks,thm:gn_ipls} that the log-posterior without the measurement is $\gnObjLin(\xSeq)$ and after introducing the measurement the log-posterior (up to a constant)
is therefore $\lmObjLin(\xSeq)$ in \cref{eq:ipls:lm:approx_cost}.
As in the earlier proofs, we conclude that the algorithms yield the same result since they minimise the same loss function in closed form.
It follows that an iteration of \ieks or \ipls for this extended state-space model is equivalent to an iteration of \lm optimisation of the corresponding cost function.
\end{proof}
In other words, we achieve an \lm-regularised version of the smoother by imposing this additional modelling assumption.
% From the perspective of the smoother
% TODO: Reflection: still shares the expected value of $\xSeq$.

%\begin{subequations}
%\begin{align}
%  \label{eq:def:ipls:lm:gnr}
%    \gnRLM(\xSeq) &=
%  \begin{pmatrix}
%    \gnR(\xSeq) \\
%    \lmRegSqrtT (\xSeq - \xHatItSeq{i})
%  \end{pmatrix} \\
%    \gnRLM(\xSeq) &: \reals^{\tsFin \dimState} \to \reals^{N + \tsFin \dimState}.
%\end{align}
%\end{subequations}

  % &=
  % \begin{pmatrix}
  %   J_{\gnR}(\xSeq) \\
  %   \lmRegSqrtT \frac{\d}{\d \xSeq} (\xSeq - \xHatItSeq{i})
  % \end{pmatrix}
  % \nonumber \\

%\begin{subequations}
%\begin{align}
%    \gnRLM'(\xSeq) &= \nonumber \\
%    &= \begin{pmatrix}
%    \gnR'(\xSeq) \\
%    \lmRegSqrtT \frac{\d}{\d \xSeq} (\xSeq - \xHatItSeq{i})
%  \end{pmatrix}
%    = \begin{pmatrix}
%    \gnR'(\xSeq) \\
%    \lmRegSqrtT
%  \end{pmatrix}
%  \\
%  \gnRLM'(\xSeq) &: \reals^{\tsFin \dimState} \to \reals^{N + \tsFin \dimState \times \tsFin \dimState}.
%\end{align}
%\end{subequations}

% the last term of \cref{eq:pls:lm:cost_fn:lin} can be written as
%
% \begin{align}
%   &\lmRegParamIt{i} (\xSeq - \xHatItSeq{i})^{\top} \left[ \regMat^{(i)}\right]^{-1} (\xSeq - \xHatItSeq{i})
%   \nonumber \\
%   =& \sum_{k=1}^{\tsFin} (\xSeq - \xHatIt{i})^{\top} \left[ (\lmRegParamIt{i})^{-1} \regMat_{\ts}^{(i)} \right]^{-1} (\xSeq - \xHatIt{i}).
% \label{eq:cost_fn:lm:block_diag_term}
% \end{align}
%Comparing this to the original cost function in \cref{eq:pls:cost_fn} we note that


==> content/_our_method/our_method.tex <==
\section{\lmIpls}
\input{content/our_method/gn_ipls.tex}
\input{content/our_method/lm_reg_thm.tex}
\input{content/our_method/line_search.tex}


==> content/ack.tex <==
 \section{Acknowledgements}
 \noindent This work was supported by the Wallenberg AI, Autonomous Systems and Software Program (WASP) funded by the Knut and Alice Wallenberg Foundation.

==> content/algs/algorithms.tex <==
\input{content/algs/lm_alg.tex}
\input{content/algs/ls_alg.tex}


==> content/background/background.tex <==
\section{Background}
\input{content/background/high_level.tex}
\input{content/background/gn_ieks.tex}


==> content/background/gn_ieks_thm_proof.tex <==
At each iteration the \gn algorithm linearises $\gnIeksObj(\xSeq)$ in \cref{eq:gn_ieks:cost_fn} with a first-order Taylor expansion around the current estimate $\xHatItSeq{i}$ and computes the next estimate $\xHatItSeq{i+1}$
as the closed form solution of the linearised objective.
The \ieks performs iterative smoothing of the state-space model in \cref{eq:def:state_space_model} by linearising it, also using first-order Taylor expansion around $\xHatItSeq{i}$ and analytically computing the next estimate $\xHatItSeq{i+1}$ with \rts smoothing.

The proof of Prop. \ref{thm:gn_ieks} can be separated into three parts:
First, constructing $\gnR(\xSeq)$ for the cost function in \cref{eq:gn_ieks:cost_fn} and linearising it around $\xHatItSeq{i}$ to obtain $\gnObjLin(\xSeq)$.
Second, linearising the state-space model, which for the \ieks is done with a first-order Taylor expansion around the estimated means $\xHatItSeq{i}$ from the previous iteration.
Third, noting that $\gnObjLin(\xSeq)$ is the negative log-posterior of the linearised state-space model in \cref{eq:def:lin:state_space_model} (up to a constant).
Then, since the \gn algorithm minimises $\gnObjLin$ in closed form, whereas the \ieks minimises the negative log-posterior, it follows that $\xHatItSeq{i}$ must be identical for both algorithms,
making them equivalent.
%both the \gn algorithm and the \ieks work by iteratively defining an approximate problem, for which they compute a closed form solution to obtain the next iterate.
%Since both approximations result in the same minimisation problem, the algorithms must be equivalent.

\begin{proof}
Let us identify the approximate cost function $\gnObjLin(\xSeq)$ that \gn would minimise in each iteration.
The first step is to write the cost function in \cref{eq:gn_ieks:cost_fn} on the \gn form in \cref{eq:gn:problem_form}.
With state and measurements collected into a single vector
\begin{equation}
  \label{eq:gn_ieks:aug_obs}
  \augObsIeks(\xSeq) = \begin{pmatrix}
    \x_1 - \priorMean \\
    \vdots \\
    \x_{\tsFin} - f_{\tsFin-1}(\x_{\tsFin-1}) \\
    \meas_1 - h_1(\x_1) \\
    \vdots \\
    \meas_{\tsFin} - h_{\tsFin}(\x_{\tsFin})
  \end{pmatrix}
\end{equation}
and the covariance matrices in one large block-diagonal matrix
$\augQIeksInv = \diag(\priorCov^{-1}, \procCov^{-1}, \dots, \procCov_{\tsFin-1}^{-1}, \measCov_{1}^{-1}, \dots, \measCov_{\tsFin}^{-1})$,
the cost function in \cref{eq:gn_ieks:cost_fn} can be expressed on a quadratic form

\begin{equation}
  \label{eq:gn_ieks:cost_compact}
  \gnIeksObj(\xSeq) = \frac{1}{2} \gnR(\xSeq)^{\top} \gnR(\xSeq),
\end{equation}
with $\gnR(\xSeq) = \augQIeksInvSqrtT \augObsIeks(\xSeq)$.
Here we use $\augQIeksInvSqrt$ to denote the square root of $\augQIeksInv$ such that $\augQIeksInvSqrt\augQIeksInvSqrtT = \augQIeksInv$.

The approximate objective is defined by the first order expansion
$\gnRLin(\xSeq) = \augQIeksInvSqrtT \augObsIeksApprox(\xSeq)$, where
\begin{small}
\begin{align}
  \label{eq:gn_ieks:aug_obs_approx}
  \augObsIeksApprox(\xSeq) &= \nonumber \\
                      &\begin{pmatrix}
               \x_1 - \priorMean \\
               \x_2 - \left( \procA_{1}(\xHatIt{i}_1) \x_1 + \procB_{1}(\xHatIt{i}_1) \right ) \\
               \vdots \\
               \x_{\tsFin} - \left( \procA_{\tsFin-1}(\xHatIt{i}_{\tsFin-1}) \x_{\tsFin-1} + \procB_{\tsFin-1}(\xHatIt{i}_{\tsFin-1}) \right ) \\
               \meas_1 - \left( \measH_{1}(\xHatIt{i}_1) \x_1 + \measC_{1}(\xHatIt{i}_1) \right) \\
               \vdots \\
               \meas_{\tsFin} - \left( \measH_{\tsFin}(\xHatIt{i}_{\tsFin}) \x_{\tsFin} + \measC_{\tsFin}(\xHatIt{i}_{\tsFin}) \right)
             \end{pmatrix},
\end{align}
\end{small}
the details of the derivation is given below.

The approximate \gn objective becomes
\begin{small}
\begin{equation}
  \label{eq:gn_ieks:approx_objective}
  \gnObjLin(\xSeq) = \frac{1}{2} \twoNorm{\gnRLin(\xSeq)}^2 =
  \frac{1}{2} \left(\augObsIeksApprox)\right)^{\top}(\xSeq) \augQIeksInv \augObsIeksApprox(\xSeq).
\end{equation}
\end{small}
\end{proof}


==> content/background/gn_method.tex <==
%This is why we can interpret the \ieks as finding the \map estimate and conversely,
%the \ipls as indeed the \textit{posterior} linearisation smoother.
\subsection{The Gauss--Newton (\gn) method}
It is useful to view the iterated smoothers as optimisation algorithms, by identifying a cost function that they minimise.
An important advantage with this is that it enables us to make use of more general optimisation methods, with better convergence properties.
% Formulated as a general optimisation problem, many techniques can be applied but the smoothers offer the advantage of exploiting the problem structure.

The Gauss--Newton (\gn) method \cite{num_opt}, is a well-known optimisation method which is used to solve problems on the form
\begin{align}
  \label{eq:gn:problem_form}
  \x^{*} &= \argMin{x}\, \gnObj(\x) \nonumber \\
  &=\argMin{x}\, \frac{1}{2} \twoNorm{\gnR(\x)}^2
  = \argMin{x}\, \frac{1}{2} \gnR(\x)^{\top} \gnR(\x),
\end{align}
where $\gnR(\x)$ is a given function.
Starting from an initial guess, the method iteratively finds the exact solution to the approximate objective
\begin{equation}
  \label{eq:gn:cost_fn_approx}
  \gnObjLin(\x) = \frac{1}{2} \twoNorm{\gnRLin(\x)}^2 = \frac{1}{2} \gnRLin(\x)^{\top} \gnRLin(\x),
\end{equation}
defined by the first order approximation of $\gnR(\cdot)$ around $\xHatIt{i}$
\begin{equation}
  \label{eq:gn:lin}
  \gnR(\x) \approx \gnRLin(\x) \coloneqq \gnR(\xHatIt{i}) + J_{\gnR}(\xHatIt{i}) (\x - \xHatIt{i}).
\end{equation}
Linearisation is done around the current iterate $\xHatIt{i}$ and the next iterate is the solution to the approximate problem \cref{eq:gn:cost_fn_approx} \cite{num_opt}.


==> content/background/high_level.tex <==
% Motivate iterative smoothers
% Motivate regularisation
\subsection{Linearisations used in smoothing}
\noindent All general Gaussian \rts smoothers use the linear \rts smoother.
What sets them apart is the use of different methods of linearising the state-space model.

The \eks is a well-known general Gaussian \rts smoother \cite{bayes_filter_book}.
It makes the linear approximation through an analytical linearisation.
For instance, to linearise the motion model in \cref{eq:def:state_space_model}, at time step $\ts$, it uses
\begin{subequations}
  \begin{align}
    %\label{eq:extended}
    \label{eq:ext:jacobian}
    \procA_{\ts}(\xHat_{\ts}) &= J_{\procFn_{\ts}}(\xHat_{\ts}), \\
    \label{eq:ext:offset}
    \procB_{\ts}(\xHat_{\ts}) &= \procFn_{\ts}(\xHat_{\ts}) - \procA_{\ts}(\xHat_{\ts}) \xHat_{\ts}, \\
    \label{eq:ext:cov}
    \procLinCov_{\ts}(\xHat_{\ts}) &= \vek{0},
  \end{align}
\end{subequations}
where $J_{\procFn_\ts}(\xHat)$ is the Jacobian of $\procFn_\ts$, evaluated at $\xHat$.
Linearisation is done at some estimate of the mean of the state $\xHat_{\ts}$.
For instance, the ordinary \eks uses the updated means $\xUpd{\ts}$.
%, whereas the \ieks uses the estimates from the previous iteration $\xHatIt{i}_{\ts}$.

Another category of smoothers uses \slr to form the linear approximation,
such as the unscented \rts and cubature \rts smoothers.
The \slr for $\procFn_{\ts}$ with respect to the density $p(\x_{\ts})$, with mean $\xHat_{\ts}$ and covariance $\PHat_{\ts}$, provides the parameters \cite{slr_results}
\begin{subequations}
  \begin{align}
    \label{eq:slr:jacobian}
    \procA_{\ts}(\xHat_{\ts}, \PHat_{\ts}) &= \PsiSlr{\procFn_{\ts}}^{\top} \PHat_{\ts}^{-1}, \\
    \label{eq:slr:offset}
    \procB_{\ts}(\xHat_{\ts}, \PHat_{\ts}) &= \stateBar_{\ts} - \procA_{\ts} \xHat_{\ts}, \\
    \label{eq:slr:cov}
    \procLinCov_{\ts}(\xHat_{\ts}, \PHat_{\ts}) &= \PhiSlr{\procFn_{\ts}} - \procA_{\ts}  \PHat_{\ts} \procA_{\ts}^{\top},
  \end{align}
\end{subequations}
where
\begin{align}
  \label{eq:slr:moments}
  %\label{eq:slr:z_bar}
  \stateBar_{\ts} &=
  %\expect{\procFn_{\ts}(\x_{\ts})} =
  \int \procFn_{\ts}(\x_{\ts}) p(\x_{\ts}) \d\x_{\ts} \nonumber \\
  %\label{eq:slr:psi}
  \PsiSlr{\procFn_{\ts}}  &=
  %\cov{\x_{\ts}}{\procFn_{\ts}(\x_{\ts})} =
  \int (\x_{\ts} - \xHat_{\ts})(\procFn_{\ts}(\x_{\ts}) - \stateBar_{\ts})^{\top} p(\x_{\ts}) \d\x_{\ts} \nonumber \\
  %\label{eq:slr:phi}
  \PhiSlr{\procFn_{\ts}} &=
  %\cov{\procFn_{\ts}(\x_{\ts})}{\procFn_{\ts}(\x_{\ts})} =
  \int (\procFn_{\ts}(\x_{\ts}) - \stateBar_{\ts})(\procFn_{\ts}(\x_{\ts}) - \stateBar_{\ts})^{\top} p(\x_{\ts}) \d\x_{\ts}.
\end{align}
When the linearisation is done with respect to a distribution $p(\x_{\ts}) = \normal(\x_{\ts}; \xHat_{\ts}, \PHat_{\ts})$,
the \slr approximation depends on both the mean $\xHat_{\ts}$ and covariance $\PHat_{\ts}$.
The moments in \cref{eq:slr:moments} are not tractable for a general function $\procFn_{\ts}$
and some form of approximation is needed,
such as a Monte Carlo method or, more commonly, a sigma point method \cite{seq_monte_carlo,bayes_filter_book}.

% Linearisation region
For non-iterative methods such as the \eks, the linearisation is done at the predicted and filtered estimates for both the filtering and smoothing passes.
With non-linear motion or measurement models, the risk is that the linearisation is a poor fit for the models over the region of interest.
Furthermore, the choice of linearisation point based on the predicted mean $\xPred{\ts}$ is not informed by the measurements $\meas_{\ts:\tsFin}$.
%In effect, they select the parameters $\ThetaSeq$ with respect to the predicted and filtered estimates of the states.
Previous work has noted that the approximation is sensitive to the linearisation point when the model is non-linear and the measurement noise is low \cite{prlf_bad_low_error}.

In the posterior linearisation approach \cite{pls}, we choose the optimal linearisation given the sequence of measurements and the resulting mean square error.
For the motion model in \cref{eq:def:state_space_model}, at time step $\ts$, we have
\begin{subequations}
\begin{align}
  \label{eq:linear_obj}
  &(\procA_{\ts}, \procB_{\ts}) = \underset{\procA_{\ts}^+, \procB_{\ts}^+}{\min\,} \expect{\twoNorm{\procFn_{\ts}(\x_{\ts}) - \procA_{\ts}^+ \x_{\ts} - \procB_{\ts}^+}^2  \mid \measSeq}, \\
  &\procLinCov_{\ts} = \nonumber \\
  \label{eq:linear_obj:error_cov}
  &\expect{
    \left( \procFn_{\ts}(\x_{\ts}) - \procA_{\ts} \x_{\ts} - \procB_{\ts} \right)
    \left( \procFn_{\ts}(\x_{\ts}) - \procA_{\ts} \x_{\ts} - \procB_{\ts} \right)^{\top} \mid \measSeq
  }.
\end{align}
\end{subequations}
However, we cannot directly select parameters with respect to the unknown true posterior distribution.
% The intuition is that, with a low-noise measurement, the posterior \pdf will be narrow and any linearisation done with respect to to the prior distribution will risk being inaccurate for the region where the posterior is large.
%This can be seen as linearising around the prior mean, rather than the posterior.

Iterative smoothers take this insight into account to improve estimation performance.
By iteratively refining the linearisation in \cref{eq:def:lin:state_space_model}, the algorithms improve the estimates by using successively better linearisations.
Given estimates of the posterior moments $\xHatItSeq{i}, \PHatItSeq{i}$, we obtain a new linear approximation $\affAppParam{i+1}$,
from which new estimates of the moments $\xHatItSeq{i+1}, \PHatItSeq{i+1}$ are obtained using \rts smoothing \cite{bayes_filter_book}.
In summary, the following two-step process is iterated:
\begin{align}
  \label{eq:iterative_smoothers:iter}
  \affAppParam{i+1} &= \text{Linearisation}\left(\xHatItSeq{i}, \PHatItSeq{i}\right) \nonumber \\
  \left(\xHatItSeq{i+1}, \PHatItSeq{i+1}\right) &= \text{\rts smoother}\left(\affAppParam{i+1}, \measSeq \right).
\end{align}
The initial estimates of the moments are commonly, but not necessarily, the output of the corresponding non-iterative smoother.
Hopefully, with every iteration, the estimates of the posterior grow closer to the true posterior until the linearisation point is chosen with respect to the true posterior distribution.

% One or two paragraphs?
The \ieks is a well-known iterative extension of the \eks \cite{bell_ieks}.
In the \ieks, the linearisation step in \cref{eq:iterative_smoothers:iter} is done with a first-order Taylor expansion around the estimated means $\xHatItSeq{i}$ from the previous iteration.
The \ipls is a more recent iterative smoother, first introduced in \cite{pls}.
In \ipls, $\affAppParam{i+1}$ is selected by performing \slr as in \cref{eq:slr:jacobian,eq:slr:offset,eq:slr:cov} and \cref{eq:slr:moments} with $p(\x_{\ts}) = \normal(\x_{\ts}; \xHatIt{i}_{\ts}, \PHatIt{i}_{\ts})$.

\input{content/background/gn_method.tex}
\input{content/background/lm_reg.tex}


==> content/background/linearisation.tex <==
\subsection{Affine approximations}
For completeness we include the formal definition of the analytical and \slr affine approximation for the measurement model $\measFn_{\ts}(\cdot)$ analogous to \cref{eq:ext:jacobian,eq:ext:cov} and \cref{eq:slr:jacobian,eq:slr:cov} respectively.
First, the analytical approximation used in the \ieks:
\begin{subequations}
  \begin{align}
    %\label{eq:extended}
    \label{eq:ext_meas:jacobian}
    \measH_{\ts}(\xHat_{\ts}) &= J_{\measFn_{\ts}}(\xHat_{\ts}) \\
    \label{eq:ext_meas:offset}
    \measC_{\ts}(\xHat_{\ts}) &= \measFn_{\ts}(\xHat_{\ts}) - \measH_{\ts}(\xHat_{\ts}) \xHat_{\ts} \\
    \label{eq:ext_meas:cov}
    \measLinCov_{\ts}(\xHat_{\ts}) &= \vek{0}.
  \end{align}
\end{subequations}

For \slr, the affine approximation of the measurement model is
\begin{subequations}
  \begin{align}
    \label{eq:slr_meas:jacobian}
    \measH_{\ts}(\xHat_{\ts}, \PHat_{\ts}) &= \PsiSlr{\measFn_{\ts}}^{\top} \PHat_{\ts}^{-1} \\
    \label{eq:slr_meas:offset}
    \measC_{\ts}(\xHat_{\ts}, \PHat_{\ts}) &= \stateBar_{\ts} - \measH_{\ts} \xHat_{\ts}  \ \\
    \label{eq:slr_meas:cov}
    \measLinCov_{\ts}(\xHat_{\ts}, \PHat_{\ts}) &= \PhiSlr{\measFn_{\ts}} - \genMat  \PHat_{\ts} \genMat^{\mathrm{T}},
  \end{align}
\end{subequations}
where
\begin{align}
  \label{eq:slr_meas:moments}
  %\label{eq:slr:z_bar}
  \measBar_{\ts} &=
  %\expect{\measFn_{\ts}(\x_{\ts})} =
  \int \measFn_{\ts}(\x_{\ts}) p(\x_{\ts}) \d\x_{\ts} \nonumber \\
  %\label{eq:slr:psi}
  \PsiSlr{\measFn_{\ts}}  &=
  %\cov{\x_{\ts}}{\measFn_{\ts}(\x_{\ts})} =
  \int (\x_{\ts} - \xHat_{\ts})(\measFn_{\ts}(\x_{\ts}) - \stateBar_{\ts})^{\top} p(\x_{\ts}) \d\x_{\ts} \nonumber \\
  %\label{eq:slr:phi}
  \PhiSlr{\measFn_{\ts}} &=
  %\cov{\measFn_{\ts}(\x_{\ts})}{\measFn_{\ts}(\x_{\ts})} =
  \int (\measFn_{\ts}(\x_{\ts}) - \stateBar_{\ts})(\measFn_{\ts}(\x_{\ts}) - \stateBar_{\ts})^{\top} p(\x_{\ts}) \d\x_{\ts}.
\end{align}


==> content/background/lm_reg.tex <==
% Iterative smoothers can find better trajectories by improving the estimates through more accurate linearisations.
% By the same logic, highly non-linear functions can cause a linearisation, inaccurate enough, that the sequence of estimates diverges.
\subsection{Levenberg--Marquardt regularisation}
The \gn method is not guaranteed to converge.
Instead, like many iterative methods, it can diverge or converge to a poor solution.
An extension of the \gn method with better convergence properties is the Levenberg--Marquardt method \cite{levenberg,marquardt,num_opt}.
In the \lm method, the standard cost function $\gnObj$ is extended with a regularisation term
\begin{align}
    \label{eq:lm:cost_fn}
    &\lmObj{i}(\x) = \gnObj(\x) \nonumber \\
    &+ \frac{1}{2} \lmRegParamIt{i} (\x - \xHatIt{i})^{\top} \left[ \regMat^{(i)}\right]^{-1} (\x - \xHatIt{i}),
\end{align}
where $\lmRegParamIt{i} > 0$ is an adaptable regularisation parameter and $\regMat^{(i)}$ is a sequence of positive definite regularisation matrices.
The matrices $\regMat^{(i)}$ can be selected to scale the problem suitably \cite{nonlinear_regression,num_opt}.
In this paper, we assume that these matrices are given while $\lmRegParamIt{i}$ is adapted as part of the optimisation algorithm.
The regularisation term encourages a new iterate to be close to the previous one, hopefully in a region where the approximation is acceptable.
A new iterate is accepted only if it decreases the cost function.
The level of regularisation is controlled by adapting $\lmRegParamIt{i}$ by
reducing $\lmRegParamIt{i}$ when an iterate is accepted and increasing it on rejection.
We introduce $\nu > 1$ as a parameter to control the adaptation and increase or reduce $\lmRegParamIt{i}$ with a factor $\nu$ on accepting or rejecting an iterate respectively \cite{marquardt,lm_adapt}.


==> content/exp/ct_bearings_only_noise.tex <==
We further include an analysis of the methods sensitivity to noise.
\begin{figure}[!t]
  \input{fig/ct_bearings_only_noise/fig.tikz}
  \caption{
  \label{fig:ct_bearings_only:noise}
  Smoother noise sensitivity, TODO: rerun with lower noise, and include error bars in the tikz plot.
  }
\end{figure}


==> content/exp/exp_list.tex <==
\section{Experiments}
There are two categories of experiments which are useful for the development of this project:
\begin{itemize}
  \item{
      \textbf{Backwards compatible tests:}
      The previous work include some numerical transformations.
      These experiments are useful to replicate, both as a check that the modifications yield results close to the original and as a demonstration of the correctness of the implementation.
      \begin{itemize}
        \item \citet{plf} (\plf) contains two numerical examples. Perhaps not that useful since we focus on smoothing, but good for the library effort.
        \item{\citet{pls} (\pls) has one with a ``nonstationary growth model'' combined with both a quadratic and a cubic measurement model.
        They also include an experiment for the L-scan IPLF, a modification we might want to include.
        }
      \end{itemize}
    }
  \item {
      \textbf{Robustness tests:}
      Experiments that demonstrate that the modifications indeed make for a more robust method.
      \begin{itemize}
          \item{
              \citet{damped_plf} (damped \plf) provides two experiments, they can perhaps be extended to the smoothing case.
              Specifically, the experiments are such that \iplf does not converge.
          }
          \item{\citet{lm_ieks} (\lmIeks) performs a single experiment with a coordinated turn model on a double-loop trajectory.}
          \item {Lennart has also proposed a ``tunnel'' experiment.
          The purpose of which is to create a scenario where a smoother must be able to handle both certain and uncertain measurements which we believe our method to do.
          }
      \end{itemize}
    }
\end{itemize}


==> content/exp/lm_ieks_exp_extra.tex <==
\subsubsection{Coordinated turn model with range only measurements}
The experiment setup is the same as in \cite{lm_ieks} with a true trajectory simulated from a coordinated turn model but with measurements of range only, rather than bearings.
The range measurements comes from two sensors placed at $(-1.5, 0.5)^{\top}$ and $(1, 1)^{\top}$ respectively TODO: exp details.
To see a discrepancy between the models we measure \rmse and \nees, averaged over 15 independent realisations.
The results are displayed in \cref{fig:ct:range_only:metrics}.
\begin{figure}
  \input{fig/ct_range_only_metrics/fig.tikz}
  \caption{\label{fig:ct:range_only:metrics}Simulated coordinated turn model with range only measurements. The plot shows averaged \rmse and \nees across iterations.}
\end{figure}
From these results it is clear that the \ipls methods consistently performs better, it also shows that these methods require fewer iterations to reach a good trajectory.
It should again be noted that a single iteration of the \ipls methods are more computationally expensive than their \ieks counterparts.
We have observed that the large spread in the metrics for the \ieks methods comes from the fact that they diverge for a significant number of the random realisations.

We further include an analysis of the methods sensitivity to noise.
\begin{figure}
  \input{fig/ct_range_only_noise/fig.tikz}
  \caption{
  \label{fig:ct_range_only:noise}
  Smoother noise sensitivity for CT experiment with range only measurements TODO: rerun with lower noise, and include error bars in the tikz plot.
  }
\end{figure}


==> content/exp/non_stat_growth.tex <==
\subsubsection{Non stationary growth}
We repeat the experiment in the original \ipls paper \cite{pls}, simulating data from a univariate non-stationary growth model with dynamic function:
\begin{equation}
  \procFn_{\ts}(\x_{\ts}) = 0.9 \x_{\ts} + \frac{10 \x_{\ts}}{1 + (\x_{\ts})^2} + 8 \cos (1.2 k),
\end{equation}
with a quadratic measurement model
\begin{equation}
  \measFn_{\ts}(\x_{\ts}) = \frac{(\x_{\ts})^2}{20},
\end{equation}
which is commonly used to compare how smoothers handle non-linearities and multimodalities \cite{inf_hmm};
with a true trajectory around 0 and a quadratic measurement model there is a possibility for a bimodal posterior distribution.
An example realisation is shown in \cref{fig:non_stat_growth:realisation}
\begin{figure}
  \input{fig/non_stat_growth/fig.tikz}
  \caption{\label{fig:non_stat_growth:realisation}Smoothing of a non-stationary growth model with quadratic measurements. The measurements do not contain information about the sign of the state, allowing for the possibility of a }
\end{figure}


==> content/exp/timings.tex <==
\subsection{Computational times}
We provide computational times of the algorithms, run on an AMD Ryzen 7 2700X Eight-Core Processor,
for the smoother versions, to show their relative computational efficiency in \cref{tab:method_timings}.
\input{tab/method_timings.tex}
We measured the time each smoother needed to complete a single iteration for the problem in \cref{sec:exp:ct_const_sens}, averaged over 100 independent realisations.
This method provides a rough estimate of the smoothers' relative efficiency but different realisations vary, depending on how many tries is required to find the next estimate.

==> content/exp/tunnel_simulation.tex <==
\subsubsection{Tunnel scenario}
We test the iterative smoothers in a slightly more realistic tunnel scenario.
The true trajectory is a simulated track consisting of straight paths and curves.
Measurements are range and bearing from a single sensor located at $(100, -100)^{\top}$ except for a part of the track where no measurements are available, simulating a tunnel.
TODO: Detailed exp details

The track, measurements and example trajectories from the different model is shown in \cref{fig:tunnel_sim:setup}.
\begin{figure}
  \input{fig/tunnel_sim/fig.tikz}
  \caption{\label{fig:tunnel_sim:setup}Tunnel scenario. The track consists of a sequence of straight lines and curves. In the bottom right corner of the track, there is a segment without measurements, representing a tunnel.}
\end{figure}
The challenge for the smoothers here is that the tunnel begins at a junction of curve and straight segments.


==> content/exp/tunnel_simulation_extra.tex <==
\subsubsection{Tunnel scenario metrics}
\begin{figure}
  \input{fig/tunnel_sim_metrics/fig.tikz}
  \caption{\label{fig:tunnel_sim:setup}Tunnel scenario metrics. Interestingly enough, the one method that fails to resemble the correct track is \lmIpls. However, this is very dependent on the parameters of the experiment.}
\end{figure}


==> content/intro/contribution.tex <==
% \section{Contribution}
In this paper, we present \lm regularised versions of the \ipls, called \lmIpls, as well as line-search versions \ipls, called \lsIpls.
The results concerning the \ieks were first presented in \cite{lm_ieks}. This paper is an extension of that work and contains the following contributions:
\begin{enumerate}
  \item{
      In \cref{sec:our_method:ipls}, we show that the \ipls can be interpreted as performing \gn optimisation of a sequence of cost functions.
   }
  \item{
      In \cref{sec:our_method:lm}, we show that \lm regularisation can be achieved with a simple modification of a state-space model.
  }
  \item{
      \cref{sec:our_method:line_search}, we introduce a class of smoother methods based on a line-search algorithm.
      We derive an efficient method for computing the Armijo--Wolfe conditions for an inexact line-search for the \ipls.
  }
  \item{
    In \cref{sec:our_method:lm_alg,sec:our_method:ls_alg}, we combine these results to introduce the algorithmic descriptions of the \lm-regularised smoothers \lmIeks and \lmIpls as well as the line-search smoothers \lsIeks and \lsIpls.
    Finally in \cref{sec:exp}, we demonstrate with numerical simulations the benefits of the proposed smoothers.
    %We also provide a high-quality python implementation of the methods, for convenient testing and experimentation.
  }
\end{enumerate}
% introduced the \lm-\ieks, by using the \ieks connection to Gauss-Newton optimisation.
% In this paper we build upon that work and produce a corresponding \gn result for the \ipls.
% We extend the Levenberg--Marquardt interpretation to include both the \ieks and \ipls,
% thereby proposing the \textit{Levenberg--Marquardt iterative posterior linearisation filter} (\lmIpls),
% a robust version of the \ipls method.
% In particular, we investigate performance on measurement models with both low and high noise.
%The foundation of this research is the \plf and \pls papers which introduce the iterative approach to linearisation with respect to the posterior.
%Since these methods struggle with convergence issues, we want to investigate methods which increase robustness.
%\cite{damped_plf} introduces such a modification for the \plf, a natural extension would be to do the same for the \pls.
%
%The purpose of a square root implementation is also increased robustness. This has already been outlined in \cite{masters} but adding this modification does not prevent further modifiations.
%
%It is also of interest to provide a high-quality implementation of this for use in future research.
%In such an implementation, an optional square root version of the algorithm has a natural place.
%
%Compare to other methods, e.g. \cite{lm_ieks, ip_cond_moments}.


==> content/lm_ipls/derivation_gn_ipls.tex <==
\subsection{Proof of gradient of the IPLS cost function }
\label{app:gn_ipls:grad}
Here, we provide the proof of \cref{thm:gn_ipls:cost_fn:grad}.
The gradient of the \ipls cost function in \cref{eq:ipls:gn:cost_fn} is
\begin{align*}
  \grad \gnIplsObj{i}(\xSeq) &= \frac{1}{2} \twoNorm{\gnRIt{i}(\xSeq)}^2 \\
                             &= J_{\gnRIt{i}}(\xSeq)^{\top} \gnRIt{i}(\xSeq).
\end{align*}

To compute $J_{\gnRIt{i}}(\xSeq)$, where $\gnRIt{i}$ is defined in \cref{eq:def:ipls:gnr},
we need the Jacobians of the \slr expectations $\stateBar(\cdot), \measBar(\cdot)$
(for brevity we use the shorthand $p_{\ts}(\x) = \normal(\x; \x_{\ts}, \PHatIt{i}_{\ts})$):
\begin{small}
\begin{align}
  \label{eq:ipls:proc_jacobian}
  J_{\stateBar_{\ts}}(\x_{\ts}) &= J(\expect{\procFn(\x_{\ts})}) \nonumber \\
                                &= J \left( \int \procFn(\x) p_{\ts}(\x) \d \x \right) \nonumber \\
                                &= \int \procFn(\x) J(p_{\ts}(\x)) \d \x \nonumber \\
                                &= \int \procFn(\x) (\x - \x_{\ts})^{\top} p_{\ts}(\x) \d \x \PHatItInv{i}
\end{align}
\end{small}
Here, we use equation (S-9 in \cite{damped_plf}) and note that
\begin{small}
\begin{align}
  \label{eq:ipls:zero_int}
  \int &\stateBar_{\ts}(\x_{\ts}) \left( \x - \x_{\ts} \right)^{\top} p_{\ts}(\x) \d \x \nonumber \\
       &= \stateBar_{\ts}(\x_{\ts}) \left( \int \x^{\top}  p_{\ts}(\x) \d \x - \x_{\ts}^{\top}  \int p_{\ts}(\x) \d \x \right) \nonumber \\
       &= \stateBar_{\ts}(\x_{\ts}) \left( \x_{\ts}^{\top}- \x_{\ts}^{\top} \right)
       = 0.
\end{align}
\end{small}
We substitute \cref{eq:ipls:zero_int} into the derivative in \cref{eq:ipls:proc_jacobian} to obtain
\begin{align}
  \label{eq:ipls:proc_bar:deriv}
  &J_{\stateBar_{\ts}}(\x_{\ts}) \nonumber \\
  &= \int \left( \procFn(\x) - \stateBar_{\ts}(\x_{\ts}) \right) \left( \x - \x_{\ts} \right)^{\top} p_{\ts}(\x) \d \x\ \PHatItInv{i}\nonumber \\
  &= \PsiSlr{\procFn_{\ts}}^{\top}(\x_{\ts}) \PHatItInv{i} = \procAIt{i}_{\ts}(\x_{\ts}),
\end{align}
i.e., the \slr Jacobian in \cref{eq:slr:jacobian}, based on the estimates at iteration $i$.

Analogously,
\begin{align}
  \label{eq:ipls:meas_bar:deriv}
  J_{\measBar_{\ts}}(\x_{\ts}) = \PsiSlr{\measFn_{\ts}}^{\top}(\x_{\ts}) \PHatItInv{i} = \measHIt{i}_{\ts}(\x_{\ts})
\end{align}
%
Given the definition of $\gnRIt{i}$ in \cref{eq:def:ipls:gnr}, let $\allDim = \tsFin \dimState + \tsFin \dimMeas$ and compute the Jacobian $J_{\gnRIt{i}}(\xSeq): \reals^{\tsFin \dimState} \to \reals^{\allDim \times \tsFin \dimState}$, in terms of the above Jacobians:
\begin{align}
  \label{eq:ipls:gnr:jacobian}
  J_{\gnRIt{i}}(\xSeq) &= J_{\augQIplsInvSqrtT \augObsIpls}(\xSeq)
  = \augQIplsInvSqrtT J_{\augObsIpls}(\xSeq) \nonumber \\
              &= \augQIplsInvSqrtT
              \begin{pmatrix}
                \procAIt{i}(\xSeq)\\
                \measHIt{i}(\xSeq)
              \end{pmatrix}
\end{align}
where,
\begin{align}
  \label{eq:def:ipls:proc_jacobian_seq}
  &\procAIt{i}(\xSeq) \coloneqq \nonumber \\
  &\begin{pmatrix}
    I_{\dimState} &0 &\hdots &~ &0 \\
    -\procAIt{i}_1(\x_1) &I_{\dimState} &0 &\hdots &0 \\
    0 &-\procAIt{i}_2(\x_2) &I_{\dimState} &\hdots &0 \\
    \vdots &~ &\ddots &~ &\vdots \\
    0 &~ &\dots &I_{\dimState} &0 \\
    0 &~ &\dots & -\procAIt{i}_{\tsFin-1}(\x_{\tsFin-1}) &I_{\dimState}\\
  \end{pmatrix} \nonumber \\
\end{align}
and
\begin{align}
  \label{eq:def:ipls:meas_jacobian_seq}
  &\measHIt{i}(\xSeq) \coloneqq \nonumber \\
  &- \diag \left( \measHIt{i}_1(\x_1), \measHIt{i}_2(\x_2), \dots, \measHIt{i}It{i}_{\tsFin}(\x_{\ts}) \right).
\end{align}

\subsection{Proof details of the IPLS GN connection}
\label{app:gn_ipls}
The proof of \cref{thm:gn_ipls} has a similar structure as the proof of \cref{thm:gn_ieks},
which is outlined in \cref{fig:props_overview}.
The proof requires linearising and construction of the approximative GN cost function $\gnRLin$
and \slr linearisation of the state-space model in \cref{eq:def:state_space_model}.
We then show that that this approximate GN objective corresponds to this approximate state-space model.
Here, we provide details of these steps.

The important part of the linearisation comes from \cref{thm:gn_ipls:cost_fn:grad}.
From the Jacobian $J_{\gnRIt{it}}$ we make the \gn approximation,
linearising around the current smoothed state sequence estimate $\xHatItSeq{i}$:
%\begin{scriptsize}
\begin{align}
  \label{eq:app:ipls:gnr:taylor}
  &\gnRIt{i}(\xSeq) \approx \gnRLin(\xSeq) \nonumber \\
  &= \gnRIt{i}(\xHatItSeq{i}) + J_{\gnRIt{i}}(\xHatItSeq{i}) (\xSeq - \xHatItSeq{i}) \nonumber \\
  &= \augQIplsInvSqrtT \augObsIpls(\xHatItSeq{i}) \nonumber \\
  &+ \augQIplsInvSqrtT
  \begin{pmatrix}
    \procAIt{i}(\xHatItSeq{i}) \\
    \measHIt{i}(\xHatItSeq{i})
  \end{pmatrix}
  (\xSeq - \xHatItSeq{i}) \nonumber \\
  % &= \augQIplsInvSqrtT \nonumber \\
  % &\begin{pmatrix}
  %   \xHatIt{i}_1 - \priorMean + \x_1 - \xHatIt{i}_1\\
  %   \xHatIt{i}_2 - \stateBar_1(\xHatIt{i}_1) - \procAIt{i}_{1}(\xHatIt{i}_1) (\x_1 - \xHatIt{i}_1) + (\x_2 - \xHatIt{i}_2)\\
  %   \xHatIt{i}_3 - \stateBar_2(\xHatIt{i}_2) - \procAIt{i}_{2}(\xHatIt{i}_2) (\x_2 - \xHatIt{i}_2) + (\x_3 - \xHatIt{i}_3)\\
  %   \vdots \\
  %   \xHatIt{i}_{\tsFin} - \stateBar_{\tsFin - 1}(\xHatIt{i}_{\tsFin - 1}) - \procAIt{i}_{\tsFin-1}(\xHatIt{i}_{\tsFin-1}) (\x_{\tsFin-1} - \xHatIt{i}_{\tsFin-1}) + (\x_{\tsFin} - \xHatIt{i}_{\tsFin})\\
  %   \meas_1 - \measBar_1(\xHatIt{i}_1) - \measHIt{i}_{1}(\xHatIt{i}_1) (\x_1 - \xHatIt{i}_1)\\
  %   \meas_2 - \measBar_2(\xHatIt{i}_2) - \measHIt{i}_{2}(\xHatIt{i}_2) (\x_2 - \xHatIt{i}_2)\\
  %   \vdots \\
  %   \meas_{\tsFin} - \measBar_{\tsFin}(\xHatIt{i}_{\tsFin}) - \measHIt{i}_{{\tsFin}}(\xHatIt{i}_{\tsFin}) (\x_{\tsFin} - \xHatIt{i}_{\tsFin})\\
  % \end{pmatrix} \nonumber \\
  &= \augQIplsInvSqrtT
  \underbrace{
  \begin{pmatrix}
    \x_1 - \priorMean \\
    \x_2 - \left( \procAIt{i}_{1}(\xHatIt{i}_1) \x_1 + \procB_{1}(\xHatIt{i}_1) \right ) \\
    \x_3 - \left( \procAIt{i}_{2}(\xHatIt{i}_2) \x_2 + \procB_{2}(\xHatIt{i}_2) \right ) \\
    \vdots \\
    \x_{\tsFin} - \left( \procAIt{i}_{\tsFin-1}(\xHatIt{i}_{\tsFin}) \x_{\tsFin} + \procB_{\tsFin-1}(\xHatIt{i}_{\tsFin}) \right ) \\
    \meas_1 - \left( \measHIt{i}_{1}(\xHatIt{i}_1) \x_1 + \measC_{1}(\xHatIt{i}_1) \right) \\
    \vdots \\
    \meas_{\tsFin} - \left( \measHIt{i}_{\tsFin}(\xHatIt{i}_{\tsFin}) \x_{\tsFin} + \measC_{\tsFin}(\xHatIt{i}_{\tsFin}) \right) \\
  \end{pmatrix}}_{\coloneqq \augObsIplsApprox(\xSeq)} \nonumber \\
  &= \augQIplsInvSqrtT \augObsIplsApprox(\xSeq)
\end{align}
%\end{scriptsize}
% where, in the second to last equality, we use the relation in \cref{eq:slr:offset}, that is, $\stateBar(\xHatIt{i}_{\ts}) - \procAIt{i}_{\ts}(\xHatIt{i}_{\ts}) \xHatIt{i}_{\ts} = \procB_{\ts}(\xHatIt{i}_{\ts})$.
% Analogously for the \slr linearisation of $\measFn(\cdot)$.
where, in the second to last equality, we use the relation in \cref{eq:slr:offset} to express $\gnRLin(\xSeq)$ in terms of the offsets $\procB_{1:\tsFin}(\cdot)$ and $\measC_{1:\tsFin}(\cdot)$.


==> content/lm_ipls/derivation_lm_reg_thm.tex <==
\subsection{Proof of \cref{thm:lm_rts_smoothing}}
Here we detail the three steps of the proof of \cref{thm:lm_rts_smoothing}.
In step 1 we derive the approximate \lm objective.
From \cref{eq:lm:cost_fn} we have that the \lm objective $\lmObj{i}(\xSeq)$ is the sum of the \gn objective $\gnObj(\xSeq)$ and a regularisation term.
By simply extending $\gnR(\xSeq)$ in \cref{eq:def:ipls:gnr}, we can construct
\begin{align}
  \label{eq:def:ipls:lm:gnr}
  \gnRLM{i}(\xSeq) &=
  \begin{pmatrix}
    \gnR(\xSeq) \\
    \lmRegSqrtT (\xSeq - \xHatItSeq{i})
  \end{pmatrix},
\end{align}
such that $\lmObj{i}(\xSeq) = \frac{1}{2}\twoNorm{\gnRLM{i}}^2$.

Since the regularisation term is linear in $\xSeq$, the resulting linearisation is
\begin{align}
  \gnRLM{i}(\xSeq) \approx
  \begin{pmatrix}
    \gnRLin(\xSeq) \\
    \lmRegSqrtT (\xSeq - \xHatItSeq{i})
  \end{pmatrix},
\end{align}
where we note that the approximate objective is indeed the approximate \gn objective in \cref{eq:ipls:approx_objective} with added \lm regularisation
\begin{align}
  \label{eq:ipls:lm:approx_cost}
  &\lmObjLin(\xSeq)
  = \frac{1}{2}
  \twoNorm{
  \begin{pmatrix}
    \gnRLin(\xSeq) \\
    \lmRegSqrtT (\xSeq - \xHatItSeq{i})
  \end{pmatrix}
  }^2
  \nonumber \\
                   &= \gnObjLin(\xSeq) \nonumber \\
                   &+ \frac{1}{2} \lmRegParamIt{i} (\xSeq - \xHatItSeq{i})^{\top} \left[ \regMat^{(i)}\right]^{-1} (\xSeq - \xHatItSeq{i}).
\end{align}

In step 2 we derive the negative log-posterior for the linearised state-space model with the measurement $\xHatIt{i}_{\ts}$ in \cref{eq:lm:extended_problem}.
The additional measurement will, for each timestep, contribute with a term $\frac{1}{2} \lmRegParamIt{i} (\x_{\ts} - \xHatIt{i}_{\ts})^{\top} \left[ \regMat^{(i)}_{\ts}\right]^{-1} (\x_{\ts} - \xHatIt{i}_{\ts})$ to the negative log-posterior.
All the extra measurements can be combined into a single term $\frac{1}{2} \lmRegParamIt{i} (\xSeq - \xHatItSeq{i})^{\top} \left[ \regMat^{(i)}\right]^{-1} (\xSeq - \xHatItSeq{i})$,
with the block-diagonal matrix $\regMat^{(i)} = \diag(\regMat_1^{(i)}, \regMat_2^{(i)}, \dots, \regMat_{\tsFin}^{(i)}),\, \regMat^{(i)}_{\ts} \in \reals^{\dimState \times \dimState}$.
Note that we restrict ourselves to $\regMat^{(i)}$ on this form, whereas other suitable options exist \cite{num_opt,nonlinear_regression}.
The measurement model for $\xHatItSeq{i}$ is linear in $\xSeq$ so the negative log-posterior of the approximated state-space model produced by \ieks or \ipls linearisation will be extended with this term.
%Compared to the previous posterior, this additional measurement will give rise to a term $\frac{1}{2} \lmRegParamIt{i} (\xSeq - \xHatItSeq{i})^{\top} \left[ \regMat^{(i)}\right]^{-1} (\xSeq - \xHatItSeq{i})$.
%For the particular choice of a sequence of block-diagonal regularisation matrices in the propostion formulation
%$\xHatItSeq{i}$ can be interpreted as a measurement of normally distributed $\xSeq$ with noise covariance $(\lmRegParamIt{i}^{-1}) \regMat^{(i)}_{\ts}$ (for every timestep $\ts$) as in \cref{eq:lm:extended_problem}.

In step 3 we compare the linearisations.
We know from \cref{thm:gn_ieks,thm:gn_ipls} that the log-posterior without the measurement is $\gnObjLin(\xSeq)$ and after introducing the measurement the log-posterior (up to a constant)
is therefore $\lmObjLin(\xSeq)$ in \cref{eq:ipls:lm:approx_cost}.
As in the earlier proofs, we conclude that the algorithms yield the same result since they minimise the same loss function in closed form.
It follows that an iteration of the \ieks or the \ipls for this extended state-space model is equivalent to an iteration of \lm optimisation of the corresponding cost function.

==> content/lm_ipls/gn_ipls.tex <==
\subsection{\gn cost function}
\label{sec:our_method:ipls}
\noindent Inspired by the \ieks, we seek to establish a similar connection between the \ipls and the \gn method.
To this end, we require a cost function that leads to a \gn method, corresponding to the \ipls.

A key difference between the \ieks and the \ipls is the role the covariances play.
In the \ieks, the analytical linearisation is done only with respect to the estimated means $\xHatItSeq{i}$, whereas the \slr linearisation of the \ipls is based on both the estimated means $\xHatItSeq{i}$ and covariances $\PHatItSeq{i}$.
The \ieks further assumes that the linearisation error covariances are zero, whereas the \ipls estimates them as $\procLinCovIt{i}_{\ts}$ and $\measLinCovIt{i}_{\ts}$ respectively.
These matrices appear in the approximate state-space model of \cref{eq:def:lin:state_space_model} and must therefore be included in a cost function.
The estimated covariances $\PHatItSeq{i}$ are implicitly included in the approximate state-space model, since they are used in the \slr linearisation.

The inclusion of the covariance matrices complicates the construction of a matching \gn objective, which should be on a quadratic form in the state sequence $\xSeq$ (or some function of it).
Note that the state sequence $\xSeq$ is the optimisation variable and that the solution to the optimisation problem becomes the state estimates $\xHatItSeq{i+1}$.
The matrix defining the quadratic form will depend on the (estimated means of the) state sequence $\xHatItSeq{i}$ and the cost function will also, implicitly, depend on the covariance sequence $\PHatItSeq{i}$.

To establish the link between the \gn method and \ipls, we construct a cost function for the sequence of states fixing the covariances $\procLinCovIt{i}_{1:\tsFin}$, $\measLinCovIt{i}_{1:\tsFin}$ and $\PHatItSeq{i}$:
\begin{align}
  \label{eq:ipls:gn:cost_fn}
  &\gnIplsObj{i}(\xSeq)
  = \frac{1}{2} \Big( (\x_1 - \priorMean)^{\top} \priorCov^{-1} (\x_1 - \priorMean) \nonumber \\
  &+ \sum_{\ts=1}^{\tsFin-1} (\x_{\ts+1} - \stateBar_{\ts}(\x_{\ts}))^{\top} \left(\procCov_{\ts} + \procLinCovIt{i}_{\ts} \right)^{-1} (\x_{\ts+1} - \stateBar_{\ts}(\x_{\ts})) \nonumber \\
  &+ \sum_{\ts=1}^\tsFin (\meas_{\ts} - \measBar_{\ts}(\x_{\ts}))^{\top} \left( \measCov_{\ts} + \measLinCovIt{i}_{\ts} \right)^{-1} (\meas_{\ts} - \measBar_{\ts}(\x_{\ts})) \Big),
\end{align}
where $\stateBar(\cdot), \measBar(\cdot)$ are
%calculated as in \cref{eq:slr:z_bar}, but restated here for clarity
the \slr estimated expectations:
\begin{subequations}
\begin{align}
  \label{eq:ipls:state_bar}
  \stateBar_{\ts}(\x_{\ts}) &= \int \procFn_{\ts}(\x) \normal(\x; \x_{\ts}, \PHatIt{i}_{\ts}) \d \x,\\
  \label{eq:ipls:meas_bar}
  \measBar_{\ts}(\x_{\ts}) &= \int \measFn_{\ts}(\x) \normal(\x; \x_{\ts}, \PHatIt{i}_{\ts}) \d \x,
\end{align}
\end{subequations}
% Same line to avoid a space indent
and $\procLinCovIt{i}_{\ts}, \measLinCovIt{i}_{\ts}$ are computed using \cref{eq:slr:cov} with respect to $\xHatItSeq{i}, \PHatItSeq{i}$ using $\procFn_{\ts}$ and $\measFn_{\ts}$ in \cref{eq:slr:moments} respectively.

An important property is that the cost function in \cref{eq:ipls:gn:cost_fn} depends on the most recent estimate of the sequence of covariance matrices,
both through the \slr expectations in \cref{eq:ipls:state_bar,eq:ipls:meas_bar} and through the estimated linearisation errors $\procLinCovIt{i}_{\ts}$ and $\measLinCovIt{i}_{\ts}$.

\input{content/lm_ipls/gn_ipls_thm.tex}
% \input{content/our_method/gn_ipls_interpret.tex}


==> content/lm_ipls/gn_ipls_interpret.tex <==
It is important to note that fixing the covariance sequence does not restrict the \rts smoother's solution of the approximate problem.
The previous estimates only affect the linearisation of the state-space model, which is always fixed during the actual smoothing pass, regardless of cost function.
The effect is only present across iterations where the method essentially requires a design-choice; keeping the same covariance sequence and cost function,
or updating the covariances, thereby changing to the next optimisation objective in the sequence.

By keeping $\procLinCovIt{i}_{\ts}, \measLinCovIt{i}_{\ts}$ fixed, we perform proper \gn optimisation for a cost function in the sequence.
A specific cost function in the sequence can be optimised multiple times, creating a sequence of intermediate estimates of the means sequence. When this ``inner'' loop is finished, we obtain the estimates $\xHatItSeq{i+1}, \PHatItSeq{i+1}$,
and move on to the next cost function in the sequence.

The update has two effects: it explicitly updates the estimated covariances of the linearisation errors,
and implicitly alters the \slr expectations $\stateBar, \measBar$, see \cref{eq:slr:moments}.
The method we propose allows for the choice between the two extremes of updating to the next cost function at every iteration or optimising each cost function to convergence before updating the covariances, or indeed something in between, with some arbitrary stopping criterion.


==> content/lm_ipls/gn_ipls_thm.tex <==
Before we derive the connection between \gn and \ipls we need to derive an expression for the gradient of our proposed cost function.
\begin{lemma}
  \label[lemma]{thm:gn_ipls:cost_fn:grad}
  The gradient of the \ipls cost function in \cref{eq:ipls:gn:cost_fn} is
  \begin{align}
    \label{eq:ipls:gn:cost_fn:grad}
    &\grad \gnIplsObj{i}(\xSeq) = J_{\gnRIt{i}}(\xSeq)^{\top} \gnRIt{i}(\xSeq),
  \end{align}
  where,
  \begin{align}
  J_{\gnRIt{i}}(\xSeq)^{\top}% \nonumber \\
  &= \begin{pmatrix}
    (\procAIt{i}(\xSeq))^{\top} & (\measHIt{i})(\xSeq))^{\top}
  \end{pmatrix} \augQIplsInvSqrt,
  \end{align}
where $\procAIt{i}(\xSeq)$ and $\measHIt{i}(\xSeq)$ are given by
\cref{eq:def:ipls:proc_jacobian_seq} and \cref{eq:def:ipls:meas_jacobian_seq} in the supplementary material,
which also contains the proof of \cref{thm:gn_ipls:cost_fn:grad}.
\end{lemma}

We can then go on to present the main result of this section.
\begin{prop}
  \label[prop]{thm:gn_ipls}
The output of one iteration of \gn optimisation of the cost function $\gnIplsObj{i}(\xSeq)$ in \cref{eq:ipls:gn:cost_fn}, defined by the current \gn estimate $\xHatItSeq{i}$ and the covariance matrices $\PHatItSeq{i}$, is the same as the means estimated by \rts smoothing of \cref{eq:def:state_space_model}, linearised with \slr around $\xHatItSeq{i}, \PHatItSeq{i}$, that is, one iteration of the \ipls.
%With $\PHatIt{i}_{\ts}, \procLinCovIt{i}_{\ts}, \measLinCovIt{i}_{\ts}$ fixed for all $k = 1, \dots, \tsFin$,
%\ipls inference of the state-space model in \cref{eq:def:state_space_model} is a \gn method for minimising the cost function in \cref{eq:ipls:gn:cost_fn}.
\end{prop}

\begin{proof}
The proof follows the steps outlined in \cref{fig:props_overview}.
We construct $\gnRIt{i}(\xSeq)$ such that $\gnIplsObj{i}(\xSeq) = \frac{1}{2} \twoNorm{\gnRIt{i}(\xSeq)}^2$ and then linearise $\gnRIt{i}(\xSeq)$ to form the approximate objective $\gnIplsObjLin{i}(\xSeq)$.
Secondly, the state-space model is linearised with \slr, according to the \ipls.
Finally, we compare the approximate \gn objective to the linearised state-space model and note that they correspond to the same minimisation problem.

Note that the covariance matrices $\procLinCovIt{i}_{\ts}$ and $\measLinCovIt{i}_{\ts}$ in $\gnIplsObj{i}(\xSeq)$ depend on the current estimates $\xHatItSeq{i}$ and not on the optimisation variable $\xSeq$.
Therefore, $\gnIplsObj{i}(\xSeq)$ is on the form of \cref{eq:gn:problem_form} and can be optimised with the \gn method.

We construct $\gnRIt{i}(\xSeq)$ by collecting states and measurements in a vector and group the covariance matrices in a single block diagonal matrix:
\begin{subequations}
\begin{align}
  \label{eq:def:ipls:aug_obs}
  \augObsIpls(\xSeq) &= \begin{pmatrix}
    \x_1 - \priorMean \\
    \x_2 - \stateBar_1(\x_1) \\
    \vdots \\
    \x_{\tsFin} - \stateBar_{\tsFin-1}(\x_{\tsFin-1}) \\
    \meas_1 - \measBar_1(\x_1) \\
    %\meas_2 - \measBar_2(\x_2) \\
    \vdots \\
    \meas_{\tsFin} - \measBar_{\tsFin}(\x_{\tsFin})
  \end{pmatrix}, \\
  \label{eq:def:ipls:augQ}
  \augQIplsInv &= \diag \Big( \nonumber \\
  &\priorCov^{-1}, (\procCov_1 + \procLinCovIt{i}_1)^{-1}, \dots, (\procCov_{\tsFin-1} + \procLinCovIt{i}_{\tsFin-1})^{-1},\nonumber \\
                 &(\measCov_1 + \measLinCovIt{i}_1)^{-1}, \dots, (\measCov_{\tsFin} + \measLinCovIt{i}_{\tsFin})^{-1} \Big).
\end{align}
\end{subequations}
Defining
\begin{equation}
  \label{eq:def:ipls:gnr}
  \gnRIt{i}(\xSeq) = \augQIplsInvSqrtT \augObsIpls(\xSeq),
\end{equation}
with $\augQIplsInvSqrt \augQIplsInvSqrtT = \augQIplsInv$, we confirm that
\begin{equation*}
  %\label{eq:ipls:cost_compact}
  \frac{1}{2} \twoNorm{\gnRIt{i}(\xSeq)}^2 = \augObsIpls^{\top}(\xSeq) \augQIplsInv \augObsIpls(\xSeq) = \gnIplsObj{i}(\xSeq).
\end{equation*}

Next, we linearise $\gnRIt{i}$ by computing the first-order approximation $\gnRLin$ around $\xHatItSeq{i}$
\begin{align}
  \label{eq:ipls:gnr:taylor}
  \gnRLin(\xSeq)
             &= \gnRIt{i}(\xHatItSeq{i}) + J_{\gnRIt{i}}(\xHatItSeq{i}) (\xSeq - \xHatItSeq{i}) \nonumber \\
             %&= \augQIplsInvSqrtT \augObsIpls(\xHatItSeq{i})
             %+ \augQIplsInvSqrtT J_{\augObsIpls}(\xSeq)(\xSeq - \xHatItSeq{i}) \nonumber \\
             &= \augQIplsInvSqrtT \augObsIplsApprox(\xSeq),
\end{align}
where
\begin{align*}
  &\augObsIplsApprox(\xSeq) = \nonumber \\
                      &\begin{pmatrix}
               \x_1 - \priorMean \\
               \x_2 - \left( \procAIt{i}_1(\xHatIt{i}_1) \x_1 + \procB_{1}(\xHatIt{i}_1) \right ) \\
               %\x_3 - \left( \procAIt{i}_{2}(\xHatIt{i}_2) \x_2 + \procB_{2}(\xHatIt{i}_2) \right ) \\
               \vdots \\
               \x_{\tsFin} - \left( \procAIt{i}_{\tsFin-1}(\xHatIt{i}_{\tsFin-1}) \x_{\tsFin-1} + \procB_{\tsFin-1}(\xHatIt{i}_{\tsFin-1}) \right ) \\
               \meas_1 - \left( \measHIt{i}_{1}(\xHatIt{i}_1) \x_1 + \measC_{1}(\xHatIt{i}_1) \right) \\
               \vdots \\
               \meas_{\tsFin} - \left( \measHIt{i}_{\tsFin}(\xHatIt{i}_{\tsFin}) \x_{\tsFin} + \measC_{\tsFin}(\xHatIt{i}_{\tsFin}) \right) \\
             \end{pmatrix}
\end{align*}
and $\procAIt{i}_{\ts}(\x_{\ts}), \measHIt{i}_{\ts}(\x_{\ts})$ are the \slr Jacobians of $\procFn_{\ts}, \measFn_{\ts}$ respectively,
see the supplementary material for the derivation details.

The approximate \gn objective becomes
\begin{align}
  \label{eq:ipls:approx_objective}
  &\gnIplsObjLin{i}(\xSeq) \nonumber \\
  % = \frac{1}{2} \twoNorm{ \gnRLin(\xSeq) }^2
  &= \frac{1}{2}\left(\augObsIplsApprox(\xSeq)\right)^{\top} \augQIplsInv \augObsIplsApprox(\xSeq) \left(\augObsIplsApprox(\xSeq)\right).
\end{align}
%We defined $\gnIplsObj{i}(\xSeq)$ in terms of the current estimates $\xHatItSeq{i}, \PHatItSeq{i}$.
%The next \gn iterate $\xHatItSeq{i}$ is the estimate that exactly minimises $\gnIplsObjLin{i}(\xSeq)$.
To perform one iteration of the \ipls, we instead first linearise the state-space model in \cref{eq:def:state_space_model} using \slr with respect to $\normal(\x_{\ts}; \xHatIt{i}_{\ts}, \PHatIt{i}_{\ts})$.
The resulting approximate state-space model is on the form \cref{eq:def:lin:state_space_model} with linearisation parameters $\affAppParam{i}$ selected using \cref{eq:slr:jacobian,eq:slr:offset,eq:slr:cov}.
The next iterate $\xHatItSeq{i+1}$ is computed as the closed-form output of \rts smoothing.

Examining $\gnIplsObjLin{i}(\xSeq)$, we note that it is the negative log-posterior of the \slr linearised state-space model (up to a constant).
The next \gn iterate will be the closed-form solution to this minimisation problem.
Since the two methods, \gn and \ipls, compute in a single iteration the exact solution to the same optimisation problem, their output $\xHatItSeq{i+1}$ must be the same.
\end{proof}


==> content/lm_ipls/lm_ipls.tex <==
\section{\lmIpls}
\input{content/lm_ipls/gn_ipls.tex}
\input{content/lm_ipls/lm_reg_thm.tex}
\input{content/algs/lm_alg.tex}


==> content/lm_ipls/lm_reg_thm.tex <==
\subsection{Levenberg--Marquardt regularisation}
\label{sec:our_method:lm}
\noindent The now established connection between the \ieks and \ipls and \gn optimisation makes the \lm method a promising alternative for regularisation.
\Cref{thm:lm_rts_smoothing} shows how \lm-regularisation can be achieved through smoothing of a slightly modified state-space model.
The result was shown for the \lmIeks in \cite{lm_ieks} and is here generalised to include the \lmIpls.
Similar interpretations of regularisation as extra measurements are discussed in \cite{lm_ieks_2,lm_observation},
but only for the \ieks.
%
\begin{prop}
  \label[prop]{thm:lm_rts_smoothing}
  Iterated smoothing with \ieks or \ipls (under the conditions in \cref{thm:gn_ipls}) for a state-space model as in \cref{eq:def:state_space_model}, extended with the measurement
  \begin{equation}
    \label{eq:lm:extended_problem}
    \xHatIt{i}_{\ts} = \x_{\ts} + \lmErr_{\ts},\qquad \lmErr_{\ts} \sim \normal(0, (\lmRegParamIt{i})^{-1} \regMat^{(i)}_{\ts})
  \end{equation}
  is a \gn method with the \lm-regularisation defined in \cref{eq:lm:cost_fn}, if $\regMat^{(i)}$ is a sequence of block-diagonal regularisation matrices:
  $\regMat^{(i)} = \diag(\regMat_1^{(i)}, \dots, \regMat_{\tsFin}^{(i)}),\, \regMat^{(i)}_{\ts} \in \reals^{\dimState \times \dimState}, \forall \ts = 1, \dots, \tsFin$.
\end{prop}

\begin{proof}
The proof follows the structure of the earlier proofs and we can use the results of \cref{thm:gn_ieks,thm:gn_ipls} to simplify it.
First, we construct $\gnRLM{i}(\xSeq)$ such that $\lmObj{i}(\xSeq) = \frac{1}{2} \twoNorm{\gnRLM{i}(\xSeq)}^2$ and
show that the linearisation of $\gnRLM{i}(\xSeq)$ results in an approximate objective which is $\gnObjLin(\xSeq)$ plus an extra term.
Second, we introduce the measurement in \cref{eq:lm:extended_problem} into the state-space model \cref{eq:def:state_space_model} and linearise.
Third, we confirm that the \lm optimisation and iterative smoothers solve the same minimisation problem at each iteration.
The full proof is given in the supplementary material.
\end{proof}
In other words, we achieve an \lm-regularised version of the smoother by imposing this additional modelling assumption.
% From the perspective of the smoother
% TODO: Reflection: still shares the expected value of $\xSeq$.

%\begin{subequations}
%\begin{align}
%  \label{eq:def:ipls:lm:gnr}
%    \gnRLM(\xSeq) &=
%  \begin{pmatrix}
%    \gnR(\xSeq) \\
%    \lmRegSqrtT (\xSeq - \xHatItSeq{i})
%  \end{pmatrix} \\
%    \gnRLM(\xSeq) &: \reals^{\tsFin \dimState} \to \reals^{N + \tsFin \dimState}.
%\end{align}
%\end{subequations}

  % &=
  % \begin{pmatrix}
  %   J_{\gnR}(\xSeq) \\
  %   \lmRegSqrtT \frac{\d}{\d \xSeq} (\xSeq - \xHatItSeq{i})
  % \end{pmatrix}
  % \nonumber \\

%\begin{subequations}
%\begin{align}
%    \gnRLM'(\xSeq) &= \nonumber \\
%    &= \begin{pmatrix}
%    \gnR'(\xSeq) \\
%    \lmRegSqrtT \frac{\d}{\d \xSeq} (\xSeq - \xHatItSeq{i})
%  \end{pmatrix}
%    = \begin{pmatrix}
%    \gnR'(\xSeq) \\
%    \lmRegSqrtT
%  \end{pmatrix}
%  \\
%  \gnRLM'(\xSeq) &: \reals^{\tsFin \dimState} \to \reals^{N + \tsFin \dimState \times \tsFin \dimState}.
%\end{align}
%\end{subequations}

% the last term of \cref{eq:pls:lm:cost_fn:lin} can be written as
%
% \begin{align}
%   &\lmRegParamIt{i} (\xSeq - \xHatItSeq{i})^{\top} \left[ \regMat^{(i)}\right]^{-1} (\xSeq - \xHatItSeq{i})
%   \nonumber \\
%   =& \sum_{k=1}^{\tsFin} (\xSeq - \xHatIt{i})^{\top} \left[ (\lmRegParamIt{i})^{-1} \regMat_{\ts}^{(i)} \right]^{-1} (\xSeq - \xHatIt{i}).
% \label{eq:cost_fn:lm:block_diag_term}
% \end{align}
%Comparing this to the original cost function in \cref{eq:pls:cost_fn} we note that


==> content/ls_ipls/line_search_conditions.tex <==
\subsection{Armijo and Wolfe step length conditions}
% TODO: pT grad f not guranteed to be negative.
This section provides the Armijo and Wolfe step length conditions for the \lsIpls method, see \cref{eq:def:armijo_cond,eq:def:wolfe_cond}.
An inexact line-search method only requires a sufficient decrease in the cost function, rather than finding the minimum along the search direction $\searchDirSeq{i}$.
A sufficient decrease is guaranteed by fulfilling two conditions of the cost function and its gradient at a point on the line.

The first condition is commonly referred to as the Armijo condition,
and combined they are called the Wolfe conditions or the Armijo--Wolfe conditions\cite{num_opt}.
The Armijo condition is a sufficient condition for a decreasing cost function,
whereas the Wolfe condition ensures that the step length $\alpha$ is large enough to give faster convergence.

To check the Armijo--Wolfe conditions for a certain step length $\alpha$ we need to compute the gradient of the cost function,
which comes directly from \cref{thm:gn_ipls:cost_fn:grad}.

Due to the sparseness of the Jacobian, the directional derivative can be computed more efficiently by evaluating the product
\begin{align}
  &(\searchDirSeq{i})^{\top} \grad \costFn(\xHatItSeq{i}) \nonumber \\
  &= (\searchDir{i}_{1})^{\top} \priorCov^{-1}(\xHatIt{i}_1 - \priorMean) \nonumber \\
  &+ \sum_{\ts=1}^{K-1} \left( \searchDir{i}_{\ts+1} - \procA_{\ts}(\xHatIt{i}_\ts) \searchDir{i}_{\ts} \right)^{\top} \nonumber \\
  &\hspace{1cm} \times (\procCov_{\ts} + \procLinCovIt{i}_{\ts})^{-1}(\xHatIt{i}_{\ts+1} - \stateBar_\ts(\xHatIt{i}_\ts)) \nonumber \\
  &- \sum_{\ts=1}^{K} \left( \measH_{\ts}(\xHatIt{i}_\ts) \searchDir{i}_{\ts} \right)^{\top} (\measCov_{\ts} + \measLinCovIt{i}_{\ts})^{-1}(\xHatIt{i}_{\ts+1} - \measBar_\ts(\xHatIt{i}_\ts)). \nonumber \\
\end{align}

The derivations for the gradient of the \ieks cost function are analogous,
but instead using the actual measurement and motion models and their respective analytical Jacobians.


==> content/ls_ipls/ls_ipls.tex <==
\section{\lsIpls}
%
\label{sec:our_method:line_search}
\noindent Another way to improve the \gn method is to introduce a line-search (LS) procedure to the algorithm \cite{num_opt}.
The LS version of the \ieks was described in \cite{lm_ieks} and here we extend it to the \ipls,
re-using the cost function in \cref{eq:ipls:gn:cost_fn}.
LS can be implemented by introducing a parameter $\alpha > 0$ to restrict the iterative update of the estimates.
That is, given $\xHatItSeq{i+1}$ and $\xHatItSeq{i}$,
we define $\searchDirSeq{i} = \xHatItSeq{i+1} - \xHatItSeq{i}$, and we obtain the LS update of the estimates:
\begin{equation}
  \label{eq:ls:update}
  \xHatItSeq{i+1}(\alpha) = \xHatItSeq{i} + \alpha \searchDirSeq{i}% \nonumber \\
  %\PHatItSeq{i+1}(\alpha) &= \PHatItSeq{i} + \alpha \Delta \PHatItSeq{i+1},
\end{equation}
where
\begin{equation}
  \label{eq:ls:step_length}
  \alpha = \argMin{\alpha' \in [0,1]} \gnObj^{(i)}(\xHatItSeq{i} + \alpha' \searchDirSeq{i}).
\end{equation}

\subsection{Armijo--Wolfe conditions for \lsIpls}
We can also use an inexact version of LS, where we seek a point
$\lsPoint = \xHatItSeq{i} + \alpha \searchDirSeq{i}$,
for which we only require a sufficient decrease in the cost function.
This is guaranteed by fulfilling the Armijo or Wolfe conditions \cite{num_opt}
\begin{subequations}
\begin{align}
  \label{eq:def:armijo_cond}
  \costFn(\lsPoint) \leq \costFn(\xHatItSeq{i}) + c_1 \alpha (\searchDirSeq{i})^{\top} \grad \costFn(\xHatItSeq{i}), \\
  \label{eq:def:wolfe_cond}
  (\searchDirSeq{i})^{\top} \grad \costFn(\lsPoint) \geq c_2 (\searchDirSeq{i})^{\top} \grad \costFn(\xHatItSeq{i}),
\end{align}
\end{subequations}
where $0 < c_1 < c_2 < 1$.

\begin{lemma}
  \label[lemma]{thm:ls:armijo_wolfe:ipls}
  An efficient computation of the directional derivatives for the \ipls cost function in \cref{eq:ipls:gn:cost_fn} to evaluate the Armijo--Wolfe conditions in \cref{eq:def:armijo_cond,eq:def:wolfe_cond}
  is given by
  \begin{align}
    &(\searchDirSeq{i})^{\top} \grad \costFn(\xHatItSeq{i})
    = (\searchDir{i}_{1})^{\top} \priorCov^{-1}(\xHatIt{i}_1 - \priorMean) \nonumber \\
    &+ \sum_{\ts=1}^{K-1} \left( \searchDir{i}_{\ts+1} - \procA_{\ts}(\xHatIt{i}_\ts) \searchDir{i}_{\ts} \right)^{\top} \nonumber \\
    &\hspace{1cm} \times (\procCov_{\ts} + \procLinCovIt{i}_{\ts})^{-1}(\xHatIt{i}_{\ts+1} - \stateBar_\ts(\xHatIt{i}_\ts)) \nonumber \\
    &- \sum_{\ts=1}^{K} \left( \measH_{\ts}(\xHatIt{i}_\ts) \searchDir{i}_{\ts} \right)^{\top} (\measCov_{\ts} + \measLinCovIt{i}_{\ts})^{-1}(\xHatIt{i}_{\ts+1} - \measBar_\ts(\xHatIt{i}_\ts)). \nonumber \\
  \end{align}
\end{lemma}
\begin{proof}
To evaluate the Armijo--Wolfe conditions for a certain step length $\alpha$,
we need to compute the gradient of the cost function in \cref{eq:ipls:gn:cost_fn},
which comes directly from \cref{thm:gn_ipls:cost_fn:grad}.
The derivations of the directional derivatives are in the supplementary material.
\end{proof}

By selecting a suitable estimate on a line between the previous estimate and the new one proposed by the smoothing iteration,
the methods improve, since the size of the update step is allowed to decrease for iteration updates that risk diverging.
Potentially, this could also lead to faster convergence, albeit with the extra computational demand incurred by finding a suitable $\alpha$.

\input{content/algs/ls_alg.tex}


==> one_col_content/ack.tex <==
 \section{Acknowledgements}
 \noindent This work was supported by the Wallenberg AI, Autonomous Systems and Software Program (WASP) funded by the Knut and Alice Wallenberg Foundation.

==> one_col_content/background/gn_ieks_thm_proof.tex <==
At each iteration the \gn algorithm linearises $\gnIeksObj(\xSeq)$ in \cref{eq:gn_ieks:cost_fn} with a first-order Taylor expansion around the current estimate $\xHatItSeq{i}$ and computes the next estimate $\xHatItSeq{i+1}$
as the closed form solution of the linearised objective.
The \ieks performs iterative smoothing of the state-space model in \cref{eq:def:state_space_model} by linearising it, also using first-order Taylor expansion around $\xHatItSeq{i}$ and analytically computing the next estimate $\xHatItSeq{i+1}$ with \rts smoothing.

The proof of Prop. \ref{thm:gn_ieks} can be separated into three parts:
First, constructing $\gnR(\xSeq)$ for the cost function in \cref{eq:gn_ieks:cost_fn} and linearising it around $\xHatItSeq{i}$ to obtain $\gnObjLin(\xSeq)$.
Second, linearising the state-space model, which for the \ieks is done with a first-order Taylor expansion around the estimated means $\xHatItSeq{i}$ from the previous iteration.
Third, noting that $\gnObjLin(\xSeq)$ is the negative log-posterior of the linearised state-space model in \cref{eq:def:lin:state_space_model} (up to a constant).
Then, since the \gn algorithm minimises $\gnObjLin$ in closed form, whereas the \ieks minimises the negative log-posterior, it follows that $\xHatItSeq{i}$ must be identical for both algorithms,
making them equivalent.
%both the \gn algorithm and the \ieks work by iteratively defining an approximate problem, for which they compute a closed form solution to obtain the next iterate.
%Since both approximations result in the same minimisation problem, the algorithms must be equivalent.

\begin{proof}
Let us identify the approximate cost function $\gnObjLin(\xSeq)$ that \gn would minimise in each iteration.
The first step is to write the cost function in \cref{eq:gn_ieks:cost_fn} on the \gn form in \cref{eq:gn:problem_form}.
With state and measurements collected into a single vector
\begin{equation}
  \label{eq:gn_ieks:aug_obs}
  \augObsIeks(\xSeq) = \begin{pmatrix}
    \x_1 - \priorMean \\
    \vdots \\
    \x_{\tsFin} - f_{\tsFin-1}(\x_{\tsFin-1}) \\
    \meas_1 - h_1(\x_1) \\
    \vdots \\
    \meas_{\tsFin} - h_{\tsFin}(\x_{\tsFin})
  \end{pmatrix}
\end{equation}
and the covariance matrices in one large block-diagonal matrix
$\augQIeksInv = \diag(\priorCov^{-1}, \procCov^{-1}, \dots, \procCov_{\tsFin-1}^{-1}, \measCov_{1}^{-1}, \dots, \measCov_{\tsFin}^{-1})$,
the cost function in \cref{eq:gn_ieks:cost_fn} can be expressed on a quadratic form

\begin{equation}
  \label{eq:gn_ieks:cost_compact}
  \gnIeksObj(\xSeq) = \frac{1}{2} \gnR(\xSeq)^{\top} \gnR(\xSeq),
\end{equation}
with $\gnR(\xSeq) = \augQIeksInvSqrtT \augObsIeks(\xSeq)$.
Here we use $\augQIeksInvSqrt$ to denote the square root of $\augQIeksInv$ such that $\augQIeksInvSqrt\augQIeksInvSqrtT = \augQIeksInv$.

The approximate objective is defined by the first order expansion
$\gnRLin(\xSeq) = \augQIeksInvSqrtT \augObsIeksApprox(\xSeq)$, where
\begin{small}
\begin{align}
  \label{eq:gn_ieks:aug_obs_approx}
  \augObsIeksApprox(\xSeq) &= \nonumber \\
                      &\begin{pmatrix}
               \x_1 - \priorMean \\
               \x_2 - \left( \procA_{1}(\xHatIt{i}_1) \x_1 + \procB_{1}(\xHatIt{i}_1) \right ) \\
               \vdots \\
               \x_{\tsFin} - \left( \procA_{\tsFin-1}(\xHatIt{i}_{\tsFin-1}) \x_{\tsFin-1} + \procB_{\tsFin-1}(\xHatIt{i}_{\tsFin-1}) \right ) \\
               \meas_1 - \left( \measH_{1}(\xHatIt{i}_1) \x_1 + \measC_{1}(\xHatIt{i}_1) \right) \\
               \vdots \\
               \meas_{\tsFin} - \left( \measH_{\tsFin}(\xHatIt{i}_{\tsFin}) \x_{\tsFin} + \measC_{\tsFin}(\xHatIt{i}_{\tsFin}) \right)
             \end{pmatrix},
\end{align}
\end{small}
the details of the derivation is given below.

The approximate \gn objective becomes
\begin{small}
\begin{equation}
  \label{eq:gn_ieks:approx_objective}
  \gnObjLin(\xSeq) = \frac{1}{2} \twoNorm{\gnRLin(\xSeq)}^2 =
  \frac{1}{2} \left(\augObsIeksApprox)\right)^{\top}(\xSeq) \augQIeksInv \augObsIeksApprox(\xSeq).
\end{equation}
\end{small}
\end{proof}


==> one_col_content/background/linearisation.tex <==
\subsection{Affine approximations}
For completeness we include the formal definition of the analytical and \slr affine approximation for the measurement model $\measFn_{\ts}(\cdot)$ analogous to \cref{eq:ext:jacobian,eq:ext:cov} and \cref{eq:slr:jacobian,eq:slr:cov} respectively.
First, the analytical approximation used in the \ieks:
\begin{subequations}
  \begin{align}
    %\label{eq:extended}
    \label{eq:ext_meas:jacobian}
    \measH_{\ts}(\xHat_{\ts}) &= J_{\measFn_{\ts}}(\xHat_{\ts}) \\
    \label{eq:ext_meas:offset}
    \measC_{\ts}(\xHat_{\ts}) &= \measFn_{\ts}(\xHat_{\ts}) - \measH_{\ts}(\xHat_{\ts}) \xHat_{\ts} \\
    \label{eq:ext_meas:cov}
    \measLinCov_{\ts}(\xHat_{\ts}) &= \vek{0}.
  \end{align}
\end{subequations}

For \slr, the affine approximation of the measurement model is
\begin{subequations}
  \begin{align}
    \label{eq:slr_meas:jacobian}
    \measH_{\ts}(\xHat_{\ts}, \PHat_{\ts}) &= \PsiSlr{\measFn_{\ts}}^{\top} \PHat_{\ts}^{-1} \\
    \label{eq:slr_meas:offset}
    \measC_{\ts}(\xHat_{\ts}, \PHat_{\ts}) &= \stateBar_{\ts} - \measH_{\ts} \xHat_{\ts}  \ \\
    \label{eq:slr_meas:cov}
    \measLinCov_{\ts}(\xHat_{\ts}, \PHat_{\ts}) &= \PhiSlr{\measFn_{\ts}} - \genMat  \PHat_{\ts} \genMat^{\mathrm{T}},
  \end{align}
\end{subequations}
where
\begin{align}
  \label{eq:slr_meas:moments}
  %\label{eq:slr:z_bar}
  \measBar_{\ts} &=
  %\expect{\measFn_{\ts}(\x_{\ts})} =
  \int \measFn_{\ts}(\x_{\ts}) p(\x_{\ts}) \d\x_{\ts} \nonumber \\
  %\label{eq:slr:psi}
  \PsiSlr{\measFn_{\ts}}  &=
  %\cov{\x_{\ts}}{\measFn_{\ts}(\x_{\ts})} =
  \int (\x_{\ts} - \xHat_{\ts})(\measFn_{\ts}(\x_{\ts}) - \stateBar_{\ts})^{\top} p(\x_{\ts}) \d\x_{\ts} \nonumber \\
  %\label{eq:slr:phi}
  \PhiSlr{\measFn_{\ts}} &=
  %\cov{\measFn_{\ts}(\x_{\ts})}{\measFn_{\ts}(\x_{\ts})} =
  \int (\measFn_{\ts}(\x_{\ts}) - \stateBar_{\ts})(\measFn_{\ts}(\x_{\ts}) - \stateBar_{\ts})^{\top} p(\x_{\ts}) \d\x_{\ts}.
\end{align}


==> tab/method_timings.tex <==
\begin{table}
  \caption{
    Time in seconds for a single smoother iteration in the experiment in \cref{sec:exp:ct_const_sens}.
    The times reported are the averages over 10 independent realisations.
  }
  \label{tab:method_timings}
    \begin{tabular}{l|l|l|l|l|l}
      \ieks & \lmIeks & \lsIeks & \ipls & \lmIpls & \lsIpls \\
      \hline
      0.10 & 0.38 & 0.66 & 0.63 & 1.23 & 8.47
    \end{tabular}
\end{table}
